The Correlation Between Dust and Gas Contents in Molecular Clouds

Molecular clouds are regions of dense gas and dust in space where new stars and planets are born. There is a strong correlation between the distribution of dust and molecular gas in molecular clouds. The present work focuses on the three-dimensional morphological comparisons between dust and gas within 567 molecular clouds identified in a previously published catalog. We confirm a sample of 112 molecular clouds, where the cloud morphology based on CO observations and dust observations displays good overall consistency. There are up to 334 molecular clouds whose dust distribution might be related to the distribution of gas. We are unable to find gas structures that correlate with the shape of the dust distribution in 24 molecular clouds. For the 112 molecular clouds where the dust distribution correlates very well with the distribution of gas, we use CO observational data to measure the physical properties of these molecular clouds and compare them with the results derived from dust, exploring the correlation between gas and dust in the molecular clouds. We found that the gas and dust in the molecular clouds have a fairly good linear relationship, with a gas-to-dust ratio of $\mathrm{GDR}=(2.80_{-0.34}^{+0.37})\times10^{21}\mathrm{\,cm^{-2}\, mag^{-1}}$. The ratio varies considerably among different molecular clouds. We measured the scale height of dust-CO clouds exhibiting strong correlations, finding $h_{Z} = 43.3_{-3.5}^{+4.0}\mathrm{\,pc}$.

==> catalog.tex <==
\startlongtable %\centerwidetable
%\movetableright=-1in
\begin{deluxetable*}{lrrccccccccccc}% 14 columns
    \tablecolumns{14}
    \tabletypesize{\scriptsize}
    \setlength{\tabcolsep}{0.02in}
    \tablewidth{0pt}
    \tablecaption{A Catalog of 112 Strongly Correlated Dust-CO Clouds in the Galactic Plane}
    \tablehead{
    \colhead{ID} &
    \colhead{$l$} &
    \colhead{$b$} &
    \colhead{$d_{0}$} &
    \colhead{$A_\mathrm{V}^\mathrm{min}$} &
    \colhead{$A_\mathrm{V}$} &
    \colhead{$T_\mathrm{p}$} &
    \colhead{$v_\mathrm{p}$} &
    \colhead{$\sigma_{v}$} &
    \colhead{$\Delta V$} &
    \colhead{$W_\mathrm{CO}$} &
    \colhead{$\NHI$} &
    \colhead{$N_\mathrm{H}$} &
    \colhead{$N_\mathrm{H}/A_\mathrm{V}$} \\
    \colhead{} &
    \colhead{($^\circ$)} &
    \colhead{($^\circ$)} &
    \colhead{(pc)} &
    \colhead{(mag)} &
    \colhead{(mag)} &
    \colhead{(K)} &
    \colhead{($\mathrm{km\, s^{-1}}$)}&
    \colhead{($\mathrm{km\, s^{-1}}$)} &
    \colhead{($\mathrm{km\, s^{-1}}$)} &
    \colhead{($\mathrm{K\, km\, s^{-1}}$)} &
    \colhead{($\mathrm{10^{20}\, cm^{-2}}$)} &
    \colhead{($\mathrm{10^{21}\, cm^{-2}}$)} &
    \colhead{($\mathrm{10^{21}\,cm^{-2}\, mag^{-1}}$)} \\
    \colhead{(1)} &
    \colhead{(2)} &
    \colhead{(3)} &
    \colhead{(4)} &
    \colhead{(5)} &
    \colhead{(6)} &
    \colhead{(7)} &
    \colhead{(8)} &
    \colhead{(9)} &
    \colhead{(10)} &
    \colhead{(11)} &
    \colhead{(12)} &
    \colhead{(13)} &
    \colhead{(14)}}
    \startdata
    $ 1 $ & $ 177.727 $ & $ -9.596 $ & $ 149.3 \pm 3.5 $ & $ 0.78 $ & $ 1.21 $ & $ 2.56 \pm 0.07 $ & $ 7.27 \pm 0.02 $ & $ 0.89 \pm 0.03 $ & $ 3.9 \mathrm{\,to\,} 10.4 $ & $ 5.708 \pm 1.108 $ & $ 6.640 \pm 0.002 $ & $ 2.947 \pm 0.443 $ & $ 2.437 \pm 0.412 $ \\
    $ 2 $ & $ 175.715 $ & $ -9.651 $ & $ 78.9 \pm 1.9 $ & $ 0.78 $ & $ 1.47 $ & $ 2.52 \pm 0.04 $ & $ 6.60 \pm 0.02 $ & $ 1.18 \pm 0.02 $ & $ 2.6 \mathrm{\,to\,} 10.4 $ & $ 7.450 \pm 1.019 $ & $ 7.210 \pm 0.002 $ & $ 3.701 \pm 0.408 $ & $ 2.524 \pm 0.339 $ \\
    $ 3 $ & $ 170.131 $ & $ -8.972 $ & $ 160.8 \pm 3.8 $ & $ 0.80 $ & $ 1.50 $ & $ 2.38 \pm 0.19 $ & $ 5.42 \pm 0.18 $ & $ 1.98 \pm 0.18 $ & $ -1.3 \mathrm{\,to\,} 11.7 $ & $ 11.796 \pm 1.397 $ & $ 10.200 \pm 0.003 $ & $ 5.738 \pm 0.559 $ & $ 3.834 \pm 0.476 $ \\
    $ 4 $ & $ 107.778 $ & $ -9.278 $ & $ 467.8 \pm 11.0 $ & $ 0.17 $ & $ 0.54 $ & $ 1.16 \pm 0.03 $ & $ 6.00 \pm 0.05 $ & $ 1.46 \pm 0.05 $ & $ 1.3 \mathrm{\,to\,} 10.4 $ & $ 4.232 \pm 0.593 $ & $ 4.120 \pm 0.002 $ & $ 2.105 \pm 0.237 $ & $ 3.868 \pm 0.528 $ \\
    $ 13 $ & $ -175.625 $ & $ -9.806 $ & $ 243.6 \pm 5.7 $ & $ 0.49 $ & $ 1.13 $ & $ 1.54 \pm 0.04 $ & $ 4.73 \pm 0.02 $ & $ 0.92 \pm 0.03 $ & $ 1.3 \mathrm{\,to\,} 7.8 $ & $ 3.540 \pm 0.519 $ & $ 6.720 \pm 0.001 $ & $ 2.088 \pm 0.208 $ & $ 1.842 \pm 0.232 $ \\
    $ 27 $ & $ 121.498 $ & $ -7.378 $ & $ 983.0 \pm 23.2 $ & $ 0.20 $ & $ 0.42 $ & $ 0.82 \pm 0.07 $ & $ -8.33 \pm 0.08 $ & $ 0.92 \pm 0.11 $ & $ -11.7 \mathrm{\,to\,} -5.2 $ & $ 1.886 \pm 0.363 $ & $ 3.620 \pm 0.002 $ & $ 1.116 \pm 0.145 $ & $ 2.638 \pm 0.398 $ \\
    $ 29 $ & $ 178.507 $ & $ -6.507 $ & $ 178.9 \pm 4.2 $ & $ 0.70 $ & $ 1.35 $ & $ 1.84 \pm 0.03 $ & $ 7.58 \pm 0.02 $ & $ 0.92 \pm 0.02 $ & $ 3.9 \mathrm{\,to\,} 10.4 $ & $ 4.242 \pm 0.914 $ & $ 6.140 \pm 0.002 $ & $ 2.311 \pm 0.365 $ & $ 1.718 \pm 0.302 $ \\
    $ 36 $ & $ -53.946 $ & $ -5.775 $ & $ 45.0 \pm 1.1 $ & $ 0.31 $ & $ 0.62 $ & $ 0.20 \pm 0.04 $ & $ 0.92 \pm 0.19 $ & $ 0.94 \pm 0.20 $ & $ -2.6 \mathrm{\,to\,} 3.9 $ & $ 0.474 \pm 0.140 $ & $ 5.270 \pm 0.002 $ & $ 0.717 \pm 0.056 $ & $ 1.156 \pm 0.127 $ \\
    $ 60 $ & $ -67.007 $ & $ -3.208 $ & $ 131.3 \pm 3.1 $ & $ 0.56 $ & $ 0.97 $ & $ 2.78 \pm 0.06 $ & $ -4.44 \pm 0.02 $ & $ 0.99 \pm 0.03 $ & $ -7.8 \mathrm{\,to\,} -1.3 $ & $ 6.912 \pm 0.849 $ & $ 5.590 \pm 0.002 $ & $ 3.324 \pm 0.339 $ & $ 3.435 \pm 0.439 $ \\
    $ 61 $ & $ -65.672 $ & $ -3.094 $ & $ 127.2 \pm 3.0 $ & $ 0.56 $ & $ 1.21 $ & $ 2.06 \pm 0.04 $ & $ -3.58 \pm 0.02 $ & $ 1.12 \pm 0.02 $ & $ -7.8 \mathrm{\,to\,} 0.0 $ & $ 5.771 \pm 0.813 $ & $ 6.920 \pm 0.002 $ & $ 3.000 \pm 0.325 $ & $ 2.481 \pm 0.330 $ \\
    $ 67 $ & $ -58.782 $ & $ -2.446 $ & $ 74.3 \pm 1.8 $ & $ 0.63 $ & $ 1.19 $ & $ 2.00 \pm 0.19 $ & $ -4.94 \pm 0.14 $ & $ 1.30 \pm 0.14 $ & $ -9.1 \mathrm{\,to\,} -1.3 $ & $ 6.462 \pm 0.919 $ & $ 7.130 \pm 0.002 $ & $ 3.298 \pm 0.368 $ & $ 2.761 \pm 0.374 $ \\
    $ 68 $ & $ 157.135 $ & $ -2.745 $ & $ 399.0 \pm 9.4 $ & $ 0.57 $ & $ 1.24 $ & $ 1.12 \pm 0.03 $ & $ -9.52 \pm 0.07 $ & $ 1.97 \pm 0.07 $ & $ -15.6 \mathrm{\,to\,} -3.9 $ & $ 5.524 \pm 0.548 $ & $ 11.700 \pm 0.002 $ & $ 3.379 \pm 0.219 $ & $ 2.726 \pm 0.274 $ \\
    $ 71 $ & $ 115.757 $ & $ -2.091 $ & $ 378.5 \pm 8.9 $ & $ 0.59 $ & $ 1.19 $ & $ 1.93 \pm 0.05 $ & $ -2.23 \pm 0.05 $ & $ 1.70 \pm 0.05 $ & $ -7.8 \mathrm{\,to\,} 2.6 $ & $ 8.208 \pm 0.650 $ & $ 9.320 \pm 0.002 $ & $ 4.215 \pm 0.260 $ & $ 3.530 \pm 0.348 $ \\
    $ 78 $ & $ -58.817 $ & $ -0.940 $ & $ 44.0 \pm 1.0 $ & $ 0.63 $ & $ 1.27 $ & $ 2.72 \pm 0.18 $ & $ -5.31 \pm 0.10 $ & $ 1.27 \pm 0.10 $ & $ -9.1 \mathrm{\,to\,} -1.3 $ & $ 8.633 \pm 0.961 $ & $ 9.170 \pm 0.002 $ & $ 4.370 \pm 0.384 $ & $ 3.442 \pm 0.402 $ \\
    $ 89 $ & $ -56.315 $ & $ 1.230 $ & $ 43.1 \pm 1.0 $ & $ 0.69 $ & $ 1.27 $ & $ 2.07 \pm 0.13 $ & $ -2.21 \pm 0.13 $ & $ 1.85 \pm 0.13 $ & $ -7.8 \mathrm{\,to\,} 3.9 $ & $ 9.569 \pm 0.905 $ & $ 10.300 \pm 0.002 $ & $ 4.858 \pm 0.362 $ & $ 3.826 \pm 0.410 $ \\
    $ 90 $ & $ -14.901 $ & $ 0.842 $ & $ 111.5 \pm 2.6 $ & $ 0.43 $ & $ 0.74 $ & $ 1.85 \pm 0.04 $ & $ 5.92 \pm 0.02 $ & $ 0.91 \pm 0.02 $ & $ 2.6 \mathrm{\,to\,} 9.1 $ & $ 4.243 \pm 0.919 $ & $ 6.210 \pm 0.002 $ & $ 2.318 \pm 0.368 $ & $ 3.130 \pm 0.552 $ \\
    $ 95 $ & $ 176.613 $ & $ 1.441 $ & $ 248.2 \pm 5.9 $ & $ 0.33 $ & $ 0.73 $ & $ 1.20 \pm 0.02 $ & $ 3.62 \pm 0.02 $ & $ 1.25 \pm 0.02 $ & $ 0.0 \mathrm{\,to\,} 7.8 $ & $ 3.757 \pm 0.483 $ & $ 9.190 \pm 0.002 $ & $ 2.422 \pm 0.193 $ & $ 3.338 \pm 0.370 $ \\
    $ 97 $ & $ 99.918 $ & $ 1.523 $ & $ 370.9 \pm 8.8 $ & $ 0.65 $ & $ 1.28 $ & $ 1.58 \pm 0.05 $ & $ -1.05 \pm 0.06 $ & $ 1.72 \pm 0.06 $ & $ -6.5 \mathrm{\,to\,} 5.2 $ & $ 6.806 \pm 1.269 $ & $ 13.600 \pm 0.002 $ & $ 4.082 \pm 0.508 $ & $ 3.177 \pm 0.465 $ \\
    $ 106 $ & $ -25.244 $ & $ 3.113 $ & $ 105.3 \pm 2.5 $ & $ 0.67 $ & $ 1.09 $ & $ 2.23 \pm 0.08 $ & $ 3.63 \pm 0.05 $ & $ 1.21 \pm 0.05 $ & $ 0.0 \mathrm{\,to\,} 7.8 $ & $ 6.766 \pm 0.852 $ & $ 5.670 \pm 0.002 $ & $ 3.273 \pm 0.341 $ & $ 3.007 \pm 0.389 $ \\
    $ 111 $ & $ -44.075 $ & $ 4.004 $ & $ 129.2 \pm 3.1 $ & $ 0.44 $ & $ 0.80 $ & $ 0.89 \pm 0.03 $ & $ -2.35 \pm 0.04 $ & $ 1.20 \pm 0.04 $ & $ -6.5 \mathrm{\,to\,} 1.3 $ & $ 2.665 \pm 0.445 $ & $ 4.750 \pm 0.002 $ & $ 1.541 \pm 0.178 $ & $ 1.923 \pm 0.267 $ \\
    $ 114 $ & $ -46.086 $ & $ 3.529 $ & $ 57.7 \pm 1.4 $ & $ 0.44 $ & $ 0.86 $ & $ 1.37 \pm 0.04 $ & $ -2.68 \pm 0.04 $ & $ 1.13 \pm 0.04 $ & $ -6.5 \mathrm{\,to\,} 1.3 $ & $ 3.860 \pm 0.489 $ & $ 5.230 \pm 0.002 $ & $ 2.067 \pm 0.195 $ & $ 2.399 \pm 0.292 $ \\
    $ 116 $ & $ 46.345 $ & $ 3.198 $ & $ 643.6 \pm 15.2 $ & $ 0.53 $ & $ 1.44 $ & $ 0.58 \pm 0.01 $ & $ 27.16 \pm 0.05 $ & $ 3.15 \pm 0.05 $ & $ 18.2 \mathrm{\,to\,} 36.4 $ & $ 4.585 \pm 0.628 $ & $ 16.900 \pm 0.003 $ & $ 3.524 \pm 0.251 $ & $ 2.454 \pm 0.257 $ \\
    $ 117 $ & $ 151.230 $ & $ 4.359 $ & $ 231.3 \pm 5.5 $ & $ 0.71 $ & $ 1.48 $ & $ 2.54 \pm 0.05 $ & $ 2.17 \pm 0.03 $ & $ 1.46 \pm 0.03 $ & $ -2.6 \mathrm{\,to\,} 6.5 $ & $ 9.288 \pm 1.216 $ & $ 6.300 \pm 0.002 $ & $ 4.345 \pm 0.486 $ & $ 2.933 \pm 0.398 $ \\
    $ 137 $ & $ -12.481 $ & $ 6.428 $ & $ 81.6 \pm 1.9 $ & $ 0.76 $ & $ 1.19 $ & $ 3.01 \pm 0.03 $ & $ 4.80 \pm 0.02 $ & $ 1.27 \pm 0.02 $ & $ 0.0 \mathrm{\,to\,} 9.1 $ & $ 9.574 \pm 0.943 $ & $ 9.370 \pm 0.002 $ & $ 4.767 \pm 0.377 $ & $ 3.991 \pm 0.440 $ \\
    $ 138 $ & $ -44.107 $ & $ 6.024 $ & $ 46.7 \pm 1.1 $ & $ 0.34 $ & $ 0.70 $ & $ 0.62 \pm 0.04 $ & $ 6.24 \pm 0.09 $ & $ 1.19 \pm 0.09 $ & $ 2.6 \mathrm{\,to\,} 10.4 $ & $ 1.841 \pm 0.155 $ & $ 3.160 \pm 0.002 $ & $ 1.052 \pm 0.062 $ & $ 1.514 \pm 0.147 $ \\
    $ 139 $ & $ 2.166 $ & $ 5.898 $ & $ 177.3 \pm 4.2 $ & $ 0.90 $ & $ 1.48 $ & $ 2.38 \pm 0.06 $ & $ 4.88 \pm 0.04 $ & $ 1.25 \pm 0.04 $ & $ 1.3 \mathrm{\,to\,} 9.1 $ & $ 7.429 \pm 1.931 $ & $ 7.850 \pm 0.002 $ & $ 3.757 \pm 0.772 $ & $ 2.536 \pm 0.557 $ \\
    $ 140 $ & $ -20.265 $ & $ 6.078 $ & $ 112.7 \pm 2.7 $ & $ 1.02 $ & $ 1.53 $ & $ 3.42 \pm 0.14 $ & $ 5.19 \pm 0.08 $ & $ 1.68 \pm 0.08 $ & $ 0.0 \mathrm{\,to\,} 10.4 $ & $ 14.396 \pm 1.539 $ & $ 7.280 \pm 0.003 $ & $ 6.486 \pm 0.615 $ & $ 4.249 \pm 0.519 $ \\
    $ 143 $ & $ -2.324 $ & $ 6.551 $ & $ 113.3 \pm 2.7 $ & $ 0.84 $ & $ 1.28 $ & $ 3.08 \pm 0.07 $ & $ 3.44 \pm 0.03 $ & $ 1.08 \pm 0.03 $ & $ 0.0 \mathrm{\,to\,} 6.5 $ & $ 8.326 \pm 1.655 $ & $ 6.950 \pm 0.002 $ & $ 4.026 \pm 0.662 $ & $ 3.133 \pm 0.569 $ \\
    $ 151 $ & $ 5.446 $ & $ 7.224 $ & $ 205.2 \pm 4.8 $ & $ 0.77 $ & $ 1.38 $ & $ 0.61 \pm 0.07 $ & $ 10.16 \pm 0.25 $ & $ 1.79 \pm 0.25 $ & $ 6.5 \mathrm{\,to\,} 14.3 $ & $ 2.668 \pm 0.489 $ & $ 7.170 \pm 0.002 $ & $ 1.784 \pm 0.196 $ & $ 1.297 \pm 0.174 $ \\
    $ 155 $ & $ -17.644 $ & $ 8.783 $ & $ 139.8 \pm 3.3 $ & $ 1.02 $ & $ 1.86 $ & $ 4.09 \pm 0.09 $ & $ 4.52 \pm 0.04 $ & $ 1.74 \pm 0.04 $ & $ -1.3 \mathrm{\,to\,} 10.4 $ & $ 17.829 \pm 1.648 $ & $ 10.400 \pm 0.002 $ & $ 8.172 \pm 0.659 $ & $ 4.395 \pm 0.490 $ \\
    $ 157 $ & $ -13.729 $ & $ 7.547 $ & $ 153.7 \pm 3.6 $ & $ 0.76 $ & $ 1.19 $ & $ 1.60 \pm 0.05 $ & $ 4.97 \pm 0.06 $ & $ 1.74 \pm 0.06 $ & $ 0.0 \mathrm{\,to\,} 10.4 $ & $ 6.950 \pm 1.042 $ & $ 10.200 \pm 0.003 $ & $ 3.800 \pm 0.417 $ & $ 3.182 \pm 0.426 $ \\
    $ 166 $ & $ 102.331 $ & $ 8.376 $ & $ 398.5 \pm 9.4 $ & $ 0.45 $ & $ 1.07 $ & $ 2.02 \pm 0.07 $ & $ 2.39 \pm 0.07 $ & $ 1.81 \pm 0.07 $ & $ -3.9 \mathrm{\,to\,} 7.8 $ & $ 9.180 \pm 1.004 $ & $ 9.450 \pm 0.003 $ & $ 4.617 \pm 0.402 $ & $ 4.302 \pm 0.500 $ \\
    $ 170 $ & $ -20.262 $ & $ 9.083 $ & $ 113.6 \pm 2.7 $ & $ 0.85 $ & $ 1.36 $ & $ 2.63 \pm 0.15 $ & $ 5.28 \pm 0.10 $ & $ 1.53 \pm 0.10 $ & $ 1.3 \mathrm{\,to\,} 10.4 $ & $ 10.020 \pm 1.901 $ & $ 7.610 \pm 0.002 $ & $ 4.769 \pm 0.760 $ & $ 3.505 \pm 0.620 $ \\
    $ 174 $ & $ 122.702 $ & $ 9.600 $ & $ 259.4 \pm 6.1 $ & $ 0.33 $ & $ 1.03 $ & $ 0.77 \pm 0.06 $ & $ 2.31 \pm 0.13 $ & $ 1.46 \pm 0.13 $ & $ -2.6 \mathrm{\,to\,} 6.5 $ & $ 2.827 \pm 0.629 $ & $ 5.290 \pm 0.002 $ & $ 1.660 \pm 0.252 $ & $ 1.615 \pm 0.274 $ \\
    $ 176 $ & $ -19.218 $ & $ 9.535 $ & $ 46.9 \pm 1.1 $ & $ 0.92 $ & $ 1.45 $ & $ 2.54 \pm 0.04 $ & $ 7.66 \pm 0.04 $ & $ 1.94 \pm 0.04 $ & $ 1.3 \mathrm{\,to\,} 13.0 $ & $ 12.322 \pm 1.686 $ & $ 8.870 \pm 0.002 $ & $ 5.816 \pm 0.675 $ & $ 4.008 \pm 0.558 $ \\
    $ 178 $ & $ -21.586 $ & $ 9.591 $ & $ 156.0 \pm 3.7 $ & $ 0.63 $ & $ 0.97 $ & $ 1.74 \pm 0.03 $ & $ 6.40 \pm 0.03 $ & $ 1.29 \pm 0.02 $ & $ 2.6 \mathrm{\,to\,} 10.4 $ & $ 5.622 \pm 1.369 $ & $ 6.730 \pm 0.002 $ & $ 2.922 \pm 0.548 $ & $ 3.020 \pm 0.612 $ \\
    $ 180 $ & $ 2.105 $ & $ 9.847 $ & $ 54.4 \pm 1.3 $ & $ 0.61 $ & $ 1.30 $ & $ 4.06 \pm 0.07 $ & $ 3.05 \pm 0.02 $ & $ 1.04 \pm 0.02 $ & $ 0.0 \mathrm{\,to\,} 6.5 $ & $ 10.601 \pm 1.329 $ & $ 4.710 \pm 0.002 $ & $ 4.711 \pm 0.532 $ & $ 3.624 \pm 0.495 $ \\
    $ 186 $ & $ -158.356 $ & $ -9.690 $ & $ 394.5 \pm 9.3 $ & $ 0.68 $ & $ 1.13 $ & $ 1.83 \pm 0.05 $ & $ 9.76 \pm 0.05 $ & $ 1.40 \pm 0.05 $ & $ 5.2 \mathrm{\,to\,} 14.3 $ & $ 6.395 \pm 1.158 $ & $ 11.000 \pm 0.002 $ & $ 3.658 \pm 0.463 $ & $ 3.227 \pm 0.478 $ \\
    $ 190 $ & $ -154.295 $ & $ -7.050 $ & $ 479.6 \pm 11.5 $ & $ 0.51 $ & $ 1.19 $ & $ 1.89 \pm 0.04 $ & $ 9.76 \pm 0.05 $ & $ 2.04 \pm 0.05 $ & $ 2.6 \mathrm{\,to\,} 15.6 $ & $ 9.655 \pm 1.207 $ & $ 13.200 \pm 0.003 $ & $ 5.182 \pm 0.483 $ & $ 4.339 \pm 0.524 $ \\
    $ 191 $ & $ -177.604 $ & $ -7.794 $ & $ 293.1 \pm 6.9 $ & $ 0.83 $ & $ 1.72 $ & $ 0.73 \pm 0.06 $ & $ 5.08 \pm 0.21 $ & $ 2.10 \pm 0.21 $ & $ -1.3 \mathrm{\,to\,} 10.4 $ & $ 3.820 \pm 0.653 $ & $ 13.100 \pm 0.002 $ & $ 2.838 \pm 0.261 $ & $ 1.647 \pm 0.198 $ \\
    $ 194 $ & $ 115.707 $ & $ -3.437 $ & $ 338.6 \pm 8.0 $ & $ 0.55 $ & $ 1.10 $ & $ 1.89 \pm 0.17 $ & $ -0.72 \pm 0.12 $ & $ 1.14 \pm 0.12 $ & $ -3.9 \mathrm{\,to\,} 2.6 $ & $ 5.371 \pm 0.701 $ & $ 6.310 \pm 0.002 $ & $ 2.780 \pm 0.280 $ & $ 2.519 \pm 0.320 $ \\
    $ 196 $ & $ 28.945 $ & $ -1.805 $ & $ 274.1 \pm 6.5 $ & $ 0.97 $ & $ 2.04 $ & $ 3.02 \pm 0.09 $ & $ 4.14 \pm 0.06 $ & $ 1.69 \pm 0.06 $ & $ -1.3 \mathrm{\,to\,} 9.1 $ & $ 12.737 \pm 1.263 $ & $ 8.950 \pm 0.003 $ & $ 5.990 \pm 0.505 $ & $ 2.935 \pm 0.335 $ \\
    $ 197 $ & $ 46.394 $ & $ -1.190 $ & $ 370.1 \pm 8.7 $ & $ 0.85 $ & $ 1.60 $ & $ 3.42 \pm 0.04 $ & $ 7.28 \pm 0.02 $ & $ 1.50 \pm 0.02 $ & $ 2.6 \mathrm{\,to\,} 11.7 $ & $ 12.822 \pm 1.422 $ & $ 8.280 \pm 0.002 $ & $ 5.957 \pm 0.569 $ & $ 3.717 \pm 0.456 $ \\
    $ 203 $ & $ 162.206 $ & $ 1.705 $ & $ 557.2 \pm 13.2 $ & $ 0.43 $ & $ 1.12 $ & $ 0.77 \pm 0.02 $ & $ -1.87 \pm 0.07 $ & $ 2.65 \pm 0.07 $ & $ -9.1 \mathrm{\,to\,} 5.2 $ & $ 5.091 \pm 0.605 $ & $ 12.500 \pm 0.003 $ & $ 3.286 \pm 0.242 $ & $ 2.938 \pm 0.313 $ \\
    $ 204 $ & $ 97.795 $ & $ 1.620 $ & $ 430.6 \pm 10.2 $ & $ 0.57 $ & $ 1.30 $ & $ 2.54 \pm 0.04 $ & $ 0.45 \pm 0.03 $ & $ 1.52 \pm 0.03 $ & $ -5.2 \mathrm{\,to\,} 5.2 $ & $ 9.687 \pm 1.027 $ & $ 10.400 \pm 0.002 $ & $ 4.915 \pm 0.411 $ & $ 3.781 \pm 0.430 $ \\
    $ 208 $ & $ 102.077 $ & $ 3.011 $ & $ 432.0 \pm 10.2 $ & $ 0.65 $ & $ 1.25 $ & $ 3.81 \pm 0.06 $ & $ -1.52 \pm 0.03 $ & $ 1.55 \pm 0.03 $ & $ -6.5 \mathrm{\,to\,} 3.9 $ & $ 14.795 \pm 1.326 $ & $ 9.000 \pm 0.002 $ & $ 6.818 \pm 0.531 $ & $ 5.434 \pm 0.595 $ \\
    $ 210 $ & $ 133.361 $ & $ 3.144 $ & $ 296.1 \pm 7.0 $ & $ 0.73 $ & $ 1.39 $ & $ 1.31 \pm 0.08 $ & $ -4.10 \pm 0.14 $ & $ 2.00 \pm 0.14 $ & $ -10.4 \mathrm{\,to\,} 2.6 $ & $ 6.539 \pm 0.960 $ & $ 12.300 \pm 0.002 $ & $ 3.845 \pm 0.384 $ & $ 2.765 \pm 0.349 $ \\
    $ 211 $ & $ 97.414 $ & $ 3.135 $ & $ 428.0 \pm 10.1 $ & $ 0.76 $ & $ 1.47 $ & $ 1.62 \pm 0.03 $ & $ 8.00 \pm 0.04 $ & $ 1.78 \pm 0.04 $ & $ 2.6 \mathrm{\,to\,} 13.0 $ & $ 7.182 \pm 0.710 $ & $ 7.150 \pm 0.003 $ & $ 3.588 \pm 0.284 $ & $ 2.447 \pm 0.270 $ \\
    $ 224 $ & $ 172.471 $ & $ 7.522 $ & $ 769.6 \pm 18.2 $ & $ 0.26 $ & $ 0.97 $ & $ 0.81 \pm 0.02 $ & $ 1.27 \pm 0.06 $ & $ 1.82 \pm 0.06 $ & $ -5.2 \mathrm{\,to\,} 7.8 $ & $ 3.670 \pm 0.474 $ & $ 12.500 \pm 0.002 $ & $ 2.718 \pm 0.190 $ & $ 2.810 \pm 0.292 $ \\
    $ 225 $ & $ 95.641 $ & $ 7.891 $ & $ 438.8 \pm 10.4 $ & $ 0.59 $ & $ 1.30 $ & $ 1.60 \pm 0.07 $ & $ -1.18 \pm 0.08 $ & $ 1.59 \pm 0.08 $ & $ -6.5 \mathrm{\,to\,} 3.9 $ & $ 6.378 \pm 1.506 $ & $ 11.300 \pm 0.003 $ & $ 3.681 \pm 0.603 $ & $ 2.832 \pm 0.512 $ \\
    $ 230 $ & $ 141.968 $ & $ 9.634 $ & $ 463.3 \pm 10.9 $ & $ 0.67 $ & $ 1.53 $ & $ 1.14 \pm 0.06 $ & $ 2.27 \pm 0.12 $ & $ 2.00 \pm 0.12 $ & $ -3.9 \mathrm{\,to\,} 9.1 $ & $ 5.737 \pm 0.694 $ & $ 8.300 \pm 0.003 $ & $ 3.125 \pm 0.277 $ & $ 2.047 \pm 0.240 $ \\
    $ 231 $ & $ 93.533 $ & $ 9.016 $ & $ 491.9 \pm 11.6 $ & $ 0.66 $ & $ 1.47 $ & $ 2.27 \pm 0.05 $ & $ -1.97 \pm 0.04 $ & $ 1.56 \pm 0.04 $ & $ -6.5 \mathrm{\,to\,} 2.6 $ & $ 8.832 \pm 1.374 $ & $ 7.850 \pm 0.002 $ & $ 4.318 \pm 0.550 $ & $ 2.945 \pm 0.438 $ \\
    $ 234 $ & $ -157.444 $ & $ -8.929 $ & $ 431.1 \pm 10.2 $ & $ 0.68 $ & $ 1.19 $ & $ 2.54 \pm 0.06 $ & $ 10.23 \pm 0.05 $ & $ 1.85 \pm 0.05 $ & $ 5.2 \mathrm{\,to\,} 15.6 $ & $ 11.708 \pm 1.320 $ & $ 11.700 \pm 0.002 $ & $ 5.853 \pm 0.528 $ & $ 4.901 \pm 0.581 $ \\
    $ 239 $ & $ 90.025 $ & $ -6.469 $ & $ 662.6 \pm 15.6 $ & $ 0.41 $ & $ 0.80 $ & $ 1.22 \pm 0.03 $ & $ 12.39 \pm 0.04 $ & $ 1.43 \pm 0.04 $ & $ 7.8 \mathrm{\,to\,} 16.9 $ & $ 4.367 \pm 0.459 $ & $ 5.580 \pm 0.002 $ & $ 2.305 \pm 0.184 $ & $ 2.877 \pm 0.319 $ \\
    $ 242 $ & $ -42.343 $ & $ -4.054 $ & $ 819.2 \pm 19.3 $ & $ 0.54 $ & $ 1.30 $ & $ 1.36 \pm 0.04 $ & $ -6.12 \pm 0.06 $ & $ 1.95 \pm 0.06 $ & $ -13.0 \mathrm{\,to\,} 0.0 $ & $ 6.632 \pm 0.919 $ & $ 10.800 \pm 0.003 $ & $ 3.733 \pm 0.367 $ & $ 2.871 \pm 0.359 $ \\
    $ 243 $ & $ 93.265 $ & $ -4.310 $ & $ 806.5 \pm 22.0 $ & $ 0.48 $ & $ 1.27 $ & $ 1.53 \pm 0.09 $ & $ 2.73 \pm 0.14 $ & $ 2.02 \pm 0.14 $ & $ -3.9 \mathrm{\,to\,} 9.1 $ & $ 7.706 \pm 0.687 $ & $ 11.100 \pm 0.003 $ & $ 4.192 \pm 0.275 $ & $ 3.302 \pm 0.334 $ \\
    $ 247 $ & $ -103.914 $ & $ -2.406 $ & $ 606.7 \pm 14.3 $ & $ 0.63 $ & $ 1.27 $ & $ 2.12 \pm 0.04 $ & $ 8.93 \pm 0.04 $ & $ 1.57 \pm 0.04 $ & $ 3.9 \mathrm{\,to\,} 13.0 $ & $ 8.295 \pm 0.841 $ & $ 11.700 \pm 0.002 $ & $ 4.488 \pm 0.337 $ & $ 3.534 \pm 0.380 $ \\
    $ 249 $ & $ 90.261 $ & $ -1.724 $ & $ 710.0 \pm 16.8 $ & $ 0.66 $ & $ 1.66 $ & $ 1.06 \pm 0.05 $ & $ 3.39 \pm 0.13 $ & $ 2.63 \pm 0.13 $ & $ -5.2 \mathrm{\,to\,} 11.7 $ & $ 7.002 \pm 1.020 $ & $ 18.200 \pm 0.003 $ & $ 4.621 \pm 0.408 $ & $ 2.779 \pm 0.325 $ \\
    $ 250 $ & $ 88.486 $ & $ -1.430 $ & $ 580.2 \pm 13.7 $ & $ 0.44 $ & $ 1.15 $ & $ 1.18 \pm 0.03 $ & $ 12.53 \pm 0.05 $ & $ 1.86 \pm 0.05 $ & $ 6.5 \mathrm{\,to\,} 18.2 $ & $ 5.495 \pm 0.767 $ & $ 7.740 \pm 0.003 $ & $ 2.972 \pm 0.307 $ & $ 2.587 \pm 0.333 $ \\
    $ 252 $ & $ 136.339 $ & $ -1.556 $ & $ 725.2 \pm 17.1 $ & $ 0.59 $ & $ 1.68 $ & $ 2.18 \pm 0.03 $ & $ -10.39 \pm 0.03 $ & $ 1.62 \pm 0.03 $ & $ -15.6 \mathrm{\,to\,} -5.2 $ & $ 8.854 \pm 0.741 $ & $ 10.800 \pm 0.002 $ & $ 4.622 \pm 0.296 $ & $ 2.754 \pm 0.276 $ \\
    $ 262 $ & $ 53.989 $ & $ 2.990 $ & $ 539.3 \pm 12.7 $ & $ 0.99 $ & $ 2.12 $ & $ 1.19 \pm 0.05 $ & $ 7.86 \pm 0.12 $ & $ 2.51 \pm 0.12 $ & $ 0.0 \mathrm{\,to\,} 15.6 $ & $ 7.482 \pm 1.037 $ & $ 17.000 \pm 0.003 $ & $ 4.693 \pm 0.415 $ & $ 2.218 \pm 0.260 $ \\
    $ 263 $ & $ 124.320 $ & $ 2.765 $ & $ 704.6 \pm 16.6 $ & $ 0.84 $ & $ 2.30 $ & $ 1.90 \pm 0.14 $ & $ -9.01 \pm 0.29 $ & $ 3.29 \pm 0.29 $ & $ -18.2 \mathrm{\,to\,} 0.0 $ & $ 15.586 \pm 1.328 $ & $ 16.800 \pm 0.003 $ & $ 7.914 \pm 0.531 $ & $ 3.444 \pm 0.352 $ \\
    $ 266 $ & $ -84.498 $ & $ 2.095 $ & $ 788.8 \pm 18.6 $ & $ 0.36 $ & $ 0.89 $ & $ 1.00 \pm 0.08 $ & $ -4.75 \pm 0.26 $ & $ 2.88 \pm 0.28 $ & $ -11.7 \mathrm{\,to\,} 0.0 $ & $ 6.790 \pm 0.859 $ & $ 12.300 \pm 0.003 $ & $ 3.946 \pm 0.344 $ & $ 4.424 \pm 0.514 $ \\
    $ 267 $ & $ -21.380 $ & $ 1.952 $ & $ 885.5 \pm 20.9 $ & $ 0.50 $ & $ 1.06 $ & $ 1.47 \pm 0.02 $ & $ -3.23 \pm 0.02 $ & $ 1.32 \pm 0.02 $ & $ -7.8 \mathrm{\,to\,} 1.3 $ & $ 4.847 \pm 0.523 $ & $ 8.470 \pm 0.002 $ & $ 2.786 \pm 0.209 $ & $ 2.633 \pm 0.283 $ \\
    $ 271 $ & $ 58.199 $ & $ 3.091 $ & $ 508.0 \pm 12.0 $ & $ 0.77 $ & $ 1.59 $ & $ 2.79 \pm 0.03 $ & $ 10.33 \pm 0.01 $ & $ 1.29 \pm 0.01 $ & $ 6.5 \mathrm{\,to\,} 14.3 $ & $ 8.982 \pm 1.418 $ & $ 9.270 \pm 0.001 $ & $ 4.520 \pm 0.567 $ & $ 2.848 \pm 0.419 $ \\
    $ 272 $ & $ 57.029 $ & $ 3.083 $ & $ 554.4 \pm 13.1 $ & $ 1.02 $ & $ 2.03 $ & $ 4.40 \pm 0.04 $ & $ 11.51 \pm 0.01 $ & $ 1.25 \pm 0.01 $ & $ 7.8 \mathrm{\,to\,} 15.6 $ & $ 13.718 \pm 1.228 $ & $ 8.360 \pm 0.002 $ & $ 6.323 \pm 0.491 $ & $ 3.122 \pm 0.341 $ \\
    $ 290 $ & $ -135.036 $ & $ 8.412 $ & $ 1060.3 \pm 51.8 $ & $ 0.12 $ & $ 0.38 $ & $ 0.59 \pm 0.05 $ & $ 12.40 \pm 0.19 $ & $ 1.72 \pm 0.19 $ & $ 7.8 \mathrm{\,to\,} 16.9 $ & $ 2.510 \pm 0.225 $ & $ 4.130 \pm 0.002 $ & $ 1.417 \pm 0.090 $ & $ 3.750 \pm 0.374 $ \\
    $ 291 $ & $ -143.970 $ & $ 8.642 $ & $ 1012.0 \pm 23.9 $ & $ 0.12 $ & $ 0.35 $ & $ 0.61 \pm 0.03 $ & $ 9.55 \pm 0.05 $ & $ 1.06 \pm 0.05 $ & $ 6.5 \mathrm{\,to\,} 13.0 $ & $ 1.626 \pm 0.270 $ & $ 3.820 \pm 0.002 $ & $ 1.032 \pm 0.108 $ & $ 2.969 \pm 0.385 $ \\
    $ 294 $ & $ 88.535 $ & $ -6.726 $ & $ 725.6 \pm 17.1 $ & $ 0.41 $ & $ 0.82 $ & $ 1.08 \pm 0.02 $ & $ -2.33 \pm 0.04 $ & $ 1.59 \pm 0.04 $ & $ -6.5 \mathrm{\,to\,} 2.6 $ & $ 4.271 \pm 0.332 $ & $ 7.890 \pm 0.002 $ & $ 2.497 \pm 0.133 $ & $ 3.059 \pm 0.286 $ \\
    $ 296 $ & $ 73.829 $ & $ -5.209 $ & $ 908.7 \pm 21.4 $ & $ 0.56 $ & $ 1.30 $ & $ 0.84 \pm 0.01 $ & $ 11.24 \pm 0.03 $ & $ 2.13 \pm 0.03 $ & $ 5.2 \mathrm{\,to\,} 18.2 $ & $ 4.459 \pm 0.572 $ & $ 13.500 \pm 0.003 $ & $ 3.133 \pm 0.229 $ & $ 2.410 \pm 0.256 $ \\
    $ 303 $ & $ -95.916 $ & $ -3.493 $ & $ 796.8 \pm 18.8 $ & $ 0.37 $ & $ 0.79 $ & $ 0.98 \pm 0.02 $ & $ 4.77 \pm 0.05 $ & $ 1.84 \pm 0.05 $ & $ -1.3 \mathrm{\,to\,} 10.4 $ & $ 4.541 \pm 1.001 $ & $ 12.200 \pm 0.003 $ & $ 3.037 \pm 0.400 $ & $ 3.863 \pm 0.590 $ \\
    $ 305 $ & $ -101.693 $ & $ -2.971 $ & $ 824.0 \pm 19.4 $ & $ 0.63 $ & $ 1.30 $ & $ 1.32 \pm 0.15 $ & $ 9.31 \pm 0.24 $ & $ 1.78 \pm 0.24 $ & $ 3.9 \mathrm{\,to\,} 14.3 $ & $ 5.896 \pm 0.873 $ & $ 17.700 \pm 0.003 $ & $ 4.128 \pm 0.349 $ & $ 3.176 \pm 0.363 $ \\
    $ 306 $ & $ 92.208 $ & $ -2.744 $ & $ 772.2 \pm 18.2 $ & $ 0.43 $ & $ 1.28 $ & $ 1.31 \pm 0.05 $ & $ 1.90 \pm 0.06 $ & $ 1.37 \pm 0.06 $ & $ -2.6 \mathrm{\,to\,} 6.5 $ & $ 4.495 \pm 1.011 $ & $ 9.770 \pm 0.002 $ & $ 2.775 \pm 0.405 $ & $ 2.160 \pm 0.356 $ \\
    $ 307 $ & $ 85.776 $ & $ -2.029 $ & $ 688.4 \pm 16.2 $ & $ 0.98 $ & $ 2.34 $ & $ 1.71 \pm 0.09 $ & $ 12.72 \pm 0.16 $ & $ 2.49 \pm 0.16 $ & $ 5.2 \mathrm{\,to\,} 19.5 $ & $ 10.629 \pm 0.851 $ & $ 11.300 \pm 0.003 $ & $ 5.382 \pm 0.340 $ & $ 2.297 \pm 0.229 $ \\
    $ 311 $ & $ -165.922 $ & $ -0.774 $ & $ 710.7 \pm 16.8 $ & $ 0.56 $ & $ 1.21 $ & $ 3.57 \pm 0.11 $ & $ 3.11 \pm 0.05 $ & $ 1.32 \pm 0.05 $ & $ -1.3 \mathrm{\,to\,} 7.8 $ & $ 11.800 \pm 1.390 $ & $ 15.900 \pm 0.002 $ & $ 6.310 \pm 0.556 $ & $ 5.218 \pm 0.610 $ \\
    $ 329 $ & $ 62.737 $ & $ 1.639 $ & $ 753.3 \pm 17.8 $ & $ 0.64 $ & $ 1.45 $ & $ 2.28 \pm 0.06 $ & $ 2.17 \pm 0.04 $ & $ 1.46 \pm 0.04 $ & $ -2.6 \mathrm{\,to\,} 6.5 $ & $ 8.354 \pm 0.676 $ & $ 9.950 \pm 0.002 $ & $ 4.337 \pm 0.270 $ & $ 2.988 \pm 0.296 $ \\
    $ 332 $ & $ 110.566 $ & $ 2.057 $ & $ 916.8 \pm 21.6 $ & $ 1.03 $ & $ 2.37 $ & $ 2.84 \pm 0.24 $ & $ -9.80 \pm 0.26 $ & $ 2.68 \pm 0.26 $ & $ -16.9 \mathrm{\,to\,} -1.3 $ & $ 18.975 \pm 1.571 $ & $ 17.500 \pm 0.003 $ & $ 9.340 \pm 0.628 $ & $ 3.935 \pm 0.402 $ \\
    $ 338 $ & $ 105.887 $ & $ 4.035 $ & $ 814.4 \pm 19.2 $ & $ 0.83 $ & $ 2.84 $ & $ 2.83 \pm 0.08 $ & $ -8.30 \pm 0.07 $ & $ 1.94 \pm 0.07 $ & $ -14.3 \mathrm{\,to\,} -2.6 $ & $ 13.763 \pm 1.290 $ & $ 12.300 \pm 0.002 $ & $ 6.735 \pm 0.516 $ & $ 2.370 \pm 0.257 $ \\
    $ 341 $ & $ -88.678 $ & $ 4.679 $ & $ 749.9 \pm 17.7 $ & $ 0.61 $ & $ 1.33 $ & $ 2.01 \pm 0.04 $ & $ -2.32 \pm 0.04 $ & $ 1.75 \pm 0.04 $ & $ -7.8 \mathrm{\,to\,} 3.9 $ & $ 8.795 \pm 1.260 $ & $ 8.390 \pm 0.002 $ & $ 4.357 \pm 0.504 $ & $ 3.275 \pm 0.455 $ \\
    $ 346 $ & $ -33.922 $ & $ 6.046 $ & $ 906.8 \pm 21.4 $ & $ 0.33 $ & $ 0.67 $ & $ 0.87 \pm 0.03 $ & $ -10.09 \pm 0.06 $ & $ 1.44 \pm 0.06 $ & $ -14.3 \mathrm{\,to\,} -5.2 $ & $ 3.124 \pm 0.342 $ & $ 4.560 \pm 0.003 $ & $ 1.705 \pm 0.137 $ & $ 2.564 \pm 0.285 $ \\
    $ 351 $ & $ 147.767 $ & $ 9.282 $ & $ 967.9 \pm 22.8 $ & $ 0.49 $ & $ 1.03 $ & $ 0.89 \pm 0.03 $ & $ -14.03 \pm 0.05 $ & $ 1.27 \pm 0.05 $ & $ -18.2 \mathrm{\,to\,} -10.4 $ & $ 2.835 \pm 0.535 $ & $ 6.730 \pm 0.002 $ & $ 1.807 \pm 0.214 $ & $ 1.758 \pm 0.248 $ \\
    $ 352 $ & $ 104.224 $ & $ 9.620 $ & $ 1126.4 \pm 26.6 $ & $ 0.36 $ & $ 0.92 $ & $ 1.12 \pm 0.07 $ & $ -5.08 \pm 0.13 $ & $ 1.83 \pm 0.13 $ & $ -10.4 \mathrm{\,to\,} 0.0 $ & $ 5.111 \pm 0.591 $ & $ 11.100 \pm 0.003 $ & $ 3.155 \pm 0.236 $ & $ 3.421 \pm 0.367 $ \\
    $ 354 $ & $ -140.679 $ & $ -9.626 $ & $ 987.2 \pm 27.9 $ & $ 0.66 $ & $ 1.32 $ & $ 2.72 \pm 0.06 $ & $ 12.20 \pm 0.03 $ & $ 1.41 \pm 0.03 $ & $ 7.8 \mathrm{\,to\,} 16.9 $ & $ 9.642 \pm 0.865 $ & $ 8.600 \pm 0.002 $ & $ 4.717 \pm 0.346 $ & $ 3.586 \pm 0.381 $ \\
    $ 355 $ & $ -140.924 $ & $ -8.805 $ & $ 948.5 \pm 22.4 $ & $ 0.66 $ & $ 1.25 $ & $ 2.57 \pm 0.06 $ & $ 11.98 \pm 0.04 $ & $ 1.36 \pm 0.04 $ & $ 7.8 \mathrm{\,to\,} 16.9 $ & $ 8.751 \pm 0.792 $ & $ 10.500 \pm 0.002 $ & $ 4.551 \pm 0.317 $ & $ 3.627 \pm 0.376 $ \\
    $ 356 $ & $ -139.204 $ & $ -8.005 $ & $ 1006.0 \pm 23.7 $ & $ 0.49 $ & $ 0.95 $ & $ 1.16 \pm 0.05 $ & $ 13.01 \pm 0.08 $ & $ 1.67 \pm 0.08 $ & $ 7.8 \mathrm{\,to\,} 18.2 $ & $ 4.827 \pm 0.703 $ & $ 10.300 \pm 0.002 $ & $ 2.961 \pm 0.281 $ & $ 3.109 \pm 0.380 $ \\
    $ 357 $ & $ -140.647 $ & $ -7.912 $ & $ 1062.4 \pm 25.1 $ & $ 0.54 $ & $ 1.15 $ & $ 2.03 \pm 0.11 $ & $ 11.68 \pm 0.08 $ & $ 1.21 \pm 0.07 $ & $ 7.8 \mathrm{\,to\,} 15.6 $ & $ 6.168 \pm 0.767 $ & $ 9.760 \pm 0.002 $ & $ 3.443 \pm 0.307 $ & $ 2.997 \pm 0.353 $ \\
    $ 364 $ & $ 63.567 $ & $ -3.295 $ & $ 1052.5 \pm 24.8 $ & $ 0.78 $ & $ 1.47 $ & $ 0.96 \pm 0.03 $ & $ 8.90 \pm 0.09 $ & $ 2.28 \pm 0.09 $ & $ 1.3 \mathrm{\,to\,} 15.6 $ & $ 5.459 \pm 1.005 $ & $ 20.700 \pm 0.003 $ & $ 4.254 \pm 0.402 $ & $ 2.901 \pm 0.354 $ \\
    $ 368 $ & $ 62.142 $ & $ -2.763 $ & $ 1014.3 \pm 23.9 $ & $ 0.78 $ & $ 1.48 $ & $ 0.85 \pm 0.05 $ & $ 10.56 \pm 0.17 $ & $ 2.50 \pm 0.17 $ & $ 2.6 \mathrm{\,to\,} 16.9 $ & $ 5.269 \pm 0.660 $ & $ 20.700 \pm 0.003 $ & $ 4.178 \pm 0.264 $ & $ 2.820 \pm 0.281 $ \\
    $ 370 $ & $ -169.588 $ & $ -2.201 $ & $ 1042.6 \pm 24.6 $ & $ 0.58 $ & $ 1.16 $ & $ 2.61 \pm 0.07 $ & $ 0.87 \pm 0.07 $ & $ 2.24 \pm 0.07 $ & $ -6.5 \mathrm{\,to\,} 7.8 $ & $ 14.655 \pm 1.366 $ & $ 20.600 \pm 0.002 $ & $ 7.922 \pm 0.546 $ & $ 6.806 \pm 0.703 $ \\
    $ 372 $ & $ -25.891 $ & $ -1.249 $ & $ 1063.9 \pm 25.1 $ & $ 0.83 $ & $ 1.69 $ & $ 2.07 \pm 0.09 $ & $ -12.74 \pm 0.13 $ & $ 2.64 \pm 0.13 $ & $ -20.8 \mathrm{\,to\,} -5.2 $ & $ 13.629 \pm 1.243 $ & $ 17.900 \pm 0.003 $ & $ 7.242 \pm 0.497 $ & $ 4.277 \pm 0.441 $ \\
    $ 373 $ & $ 126.634 $ & $ -0.874 $ & $ 958.9 \pm 22.6 $ & $ 0.61 $ & $ 1.13 $ & $ 3.03 \pm 0.08 $ & $ -12.57 \pm 0.08 $ & $ 2.49 \pm 0.08 $ & $ -20.8 \mathrm{\,to\,} -5.2 $ & $ 18.824 \pm 1.206 $ & $ 13.000 \pm 0.003 $ & $ 8.830 \pm 0.482 $ & $ 7.788 \pm 0.735 $ \\
    $ 378 $ & $ -34.191 $ & $ -0.415 $ & $ 1072.9 \pm 25.3 $ & $ 0.84 $ & $ 1.63 $ & $ 0.97 \pm 0.02 $ & $ -16.84 \pm 0.09 $ & $ 3.11 \pm 0.09 $ & $ -26.0 \mathrm{\,to\,} -9.1 $ & $ 7.502 \pm 0.797 $ & $ 16.500 \pm 0.004 $ & $ 4.651 \pm 0.319 $ & $ 2.849 \pm 0.294 $ \\
    $ 392 $ & $ -148.532 $ & $ 2.463 $ & $ 1204.6 \pm 28.4 $ & $ 0.30 $ & $ 0.73 $ & $ 0.94 \pm 0.03 $ & $ 7.63 \pm 0.05 $ & $ 1.67 \pm 0.05 $ & $ 2.6 \mathrm{\,to\,} 13.0 $ & $ 3.944 \pm 0.569 $ & $ 11.200 \pm 0.003 $ & $ 2.698 \pm 0.228 $ & $ 3.718 \pm 0.424 $ \\
    $ 396 $ & $ -36.186 $ & $ 5.604 $ & $ 993.8 \pm 23.5 $ & $ 0.37 $ & $ 0.68 $ & $ 0.73 \pm 0.03 $ & $ -19.39 \pm 0.06 $ & $ 1.33 \pm 0.06 $ & $ -23.4 \mathrm{\,to\,} -15.6 $ & $ 2.423 \pm 0.191 $ & $ 5.360 \pm 0.002 $ & $ 1.505 \pm 0.076 $ & $ 2.213 \pm 0.204 $ \\
    $ 397 $ & $ -52.924 $ & $ 6.425 $ & $ 1118.7 \pm 26.4 $ & $ 0.28 $ & $ 0.63 $ & $ 0.77 \pm 0.02 $ & $ -13.45 \pm 0.04 $ & $ 1.55 \pm 0.04 $ & $ -18.2 \mathrm{\,to\,} -7.8 $ & $ 2.990 \pm 0.268 $ & $ 6.510 \pm 0.003 $ & $ 1.847 \pm 0.107 $ & $ 2.909 \pm 0.280 $ \\
    $ 403 $ & $ -175.483 $ & $ -3.770 $ & $ 1482.5 \pm 113.1 $ & $ 0.41 $ & $ 1.32 $ & $ 1.23 \pm 0.02 $ & $ 2.48 \pm 0.03 $ & $ 2.04 \pm 0.03 $ & $ -3.9 \mathrm{\,to\,} 9.1 $ & $ 6.294 \pm 0.936 $ & $ 21.800 \pm 0.003 $ & $ 4.698 \pm 0.374 $ & $ 3.572 \pm 0.396 $ \\
    $ 407 $ & $ -111.299 $ & $ -4.148 $ & $ 1664.1 \pm 39.3 $ & $ 0.49 $ & $ 2.15 $ & $ 0.50 \pm 0.02 $ & $ 19.69 \pm 0.13 $ & $ 3.15 \pm 0.13 $ & $ 11.7 \mathrm{\,to\,} 27.3 $ & $ 3.913 \pm 0.423 $ & $ 22.400 \pm 0.003 $ & $ 3.805 \pm 0.169 $ & $ 1.773 \pm 0.157 $ \\
    $ 415 $ & $ -139.438 $ & $ -1.882 $ & $ 1333.6 \pm 31.5 $ & $ 0.29 $ & $ 0.68 $ & $ 1.09 \pm 0.10 $ & $ 12.38 \pm 0.20 $ & $ 1.97 \pm 0.20 $ & $ 6.5 \mathrm{\,to\,} 18.2 $ & $ 5.390 \pm 0.555 $ & $ 12.700 \pm 0.003 $ & $ 3.426 \pm 0.222 $ & $ 5.037 \pm 0.507 $ \\
    $ 422 $ & $ -17.016 $ & $ -0.636 $ & $ 1098.9 \pm 25.9 $ & $ 0.95 $ & $ 1.51 $ & $ 2.97 \pm 0.06 $ & $ -4.43 \pm 0.06 $ & $ 2.56 \pm 0.06 $ & $ -11.7 \mathrm{\,to\,} 3.9 $ & $ 19.036 \pm 1.581 $ & $ 20.400 \pm 0.003 $ & $ 9.654 \pm 0.632 $ & $ 6.387 \pm 0.645 $ \\
    $ 427 $ & $ -134.286 $ & $ -0.429 $ & $ 1316.9 \pm 31.1 $ & $ 0.66 $ & $ 1.56 $ & $ 1.75 \pm 0.02 $ & $ 16.24 \pm 0.03 $ & $ 1.94 \pm 0.03 $ & $ 10.4 \mathrm{\,to\,} 22.1 $ & $ 8.490 \pm 1.227 $ & $ 13.300 \pm 0.003 $ & $ 4.726 \pm 0.491 $ & $ 3.035 \pm 0.392 $ \\
    $ 434 $ & $ -38.664 $ & $ 1.305 $ & $ 1142.8 \pm 27.0 $ & $ 0.65 $ & $ 1.19 $ & $ 1.18 \pm 0.08 $ & $ -18.66 \pm 0.19 $ & $ 2.39 \pm 0.19 $ & $ -24.7 \mathrm{\,to\,} -11.7 $ & $ 7.006 \pm 0.980 $ & $ 14.300 \pm 0.003 $ & $ 4.232 \pm 0.392 $ & $ 3.544 \pm 0.427 $ \\
    $ 438 $ & $ 102.810 $ & $ 2.198 $ & $ 1361.8 \pm 32.1 $ & $ 0.42 $ & $ 0.74 $ & $ 1.61 \pm 0.10 $ & $ -17.81 \pm 0.16 $ & $ 2.21 \pm 0.16 $ & $ -24.7 \mathrm{\,to\,} -10.4 $ & $ 8.925 \pm 0.569 $ & $ 14.800 \pm 0.002 $ & $ 5.050 \pm 0.228 $ & $ 6.818 \pm 0.608 $ \\
    $ 450 $ & $ -120.491 $ & $ -4.545 $ & $ 1448.8 \pm 34.2 $ & $ 0.57 $ & $ 1.12 $ & $ 1.65 \pm 0.14 $ & $ 23.07 \pm 0.20 $ & $ 2.01 \pm 0.20 $ & $ 16.9 \mathrm{\,to\,} 28.6 $ & $ 8.247 \pm 0.590 $ & $ 12.600 \pm 0.003 $ & $ 4.559 \pm 0.236 $ & $ 4.075 \pm 0.378 $ \\
    $ 451 $ & $ -121.122 $ & $ -3.822 $ & $ 1435.9 \pm 33.9 $ & $ 0.57 $ & $ 1.24 $ & $ 0.70 \pm 0.05 $ & $ 19.96 \pm 0.19 $ & $ 2.35 \pm 0.19 $ & $ 14.3 \mathrm{\,to\,} 27.3 $ & $ 4.100 \pm 0.592 $ & $ 15.300 \pm 0.003 $ & $ 3.170 \pm 0.237 $ & $ 2.558 \pm 0.274 $ \\
    $ 453 $ & $ -167.335 $ & $ -3.558 $ & $ 1650.5 \pm 76.6 $ & $ 0.34 $ & $ 1.01 $ & $ 1.39 \pm 0.08 $ & $ 4.59 \pm 0.11 $ & $ 1.59 \pm 0.11 $ & $ 0.0 \mathrm{\,to\,} 9.1 $ & $ 5.499 \pm 1.259 $ & $ 16.400 \pm 0.002 $ & $ 3.839 \pm 0.504 $ & $ 3.791 \pm 0.577 $ \\
    $ 455 $ & $ -117.320 $ & $ -3.045 $ & $ 1818.0 \pm 42.9 $ & $ 0.30 $ & $ 0.89 $ & $ 0.46 \pm 0.02 $ & $ 24.01 \pm 0.10 $ & $ 2.50 \pm 0.10 $ & $ 15.6 \mathrm{\,to\,} 31.2 $ & $ 2.884 \pm 0.367 $ & $ 15.700 \pm 0.003 $ & $ 2.723 \pm 0.147 $ & $ 3.054 \pm 0.287 $ \\
    $ 480 $ & $ 156.474 $ & $ -1.610 $ & $ 1653.1 \pm 47.0 $ & $ 0.29 $ & $ 0.68 $ & $ 0.50 \pm 0.03 $ & $ -36.10 \pm 0.15 $ & $ 2.24 \pm 0.15 $ & $ -42.9 \mathrm{\,to\,} -29.9 $ & $ 2.782 \pm 0.394 $ & $ 11.300 \pm 0.002 $ & $ 2.243 \pm 0.158 $ & $ 3.297 \pm 0.344 $ \\
    $ 494 $ & $ -55.447 $ & $ 1.348 $ & $ 1813.7 \pm 58.2 $ & $ 0.45 $ & $ 1.28 $ & $ 1.99 \pm 0.17 $ & $ -28.09 \pm 0.32 $ & $ 3.34 \pm 0.32 $ & $ -36.4 \mathrm{\,to\,} -19.5 $ & $ 16.479 \pm 2.341 $ & $ 23.800 \pm 0.003 $ & $ 8.972 \pm 0.937 $ & $ 6.983 \pm 0.905 $ \\
    $ 509 $ & $ 156.277 $ & $ -0.429 $ & $ 2033.5 \pm 64.2 $ & $ 0.26 $ & $ 0.57 $ & $ 0.52 \pm 0.01 $ & $ -34.34 \pm 0.05 $ & $ 2.03 \pm 0.05 $ & $ -39.0 \mathrm{\,to\,} -28.6 $ & $ 2.614 \pm 0.433 $ & $ 14.700 \pm 0.002 $ & $ 2.516 \pm 0.173 $ & $ 4.379 \pm 0.452 $ \\
    $ 533 $ & $ 137.066 $ & $ 1.428 $ & $ 2311.3 \pm 54.5 $ & $ 0.23 $ & $ 0.59 $ & $ 0.96 \pm 0.02 $ & $ -38.27 \pm 0.07 $ & $ 2.64 \pm 0.07 $ & $ -46.8 \mathrm{\,to\,} -31.2 $ & $ 6.320 \pm 0.551 $ & $ 19.100 \pm 0.003 $ & $ 4.438 \pm 0.220 $ & $ 7.528 \pm 0.689 $ \\
    $ 548 $ & $ 123.321 $ & $ -6.529 $ & $ 2992.1 \pm 112.7 $ & $ 0.12 $ & $ 0.36 $ & $ 0.86 \pm 0.04 $ & $ -30.50 \pm 0.08 $ & $ 1.36 \pm 0.08 $ & $ -35.1 \mathrm{\,to\,} -26.0 $ & $ 2.925 \pm 0.317 $ & $ 7.130 \pm 0.002 $ & $ 1.883 \pm 0.127 $ & $ 5.190 \pm 0.531 $ \\
    $ 553 $ & $ 115.842 $ & $ -3.109 $ & $ 2954.3 \pm 107.0 $ & $ 0.17 $ & $ 0.38 $ & $ 1.17 \pm 0.06 $ & $ -0.84 \pm 0.07 $ & $ 1.21 \pm 0.07 $ & $ -5.2 \mathrm{\,to\,} 2.6 $ & $ 3.559 \pm 0.718 $ & $ 7.550 \pm 0.002 $ & $ 2.179 \pm 0.287 $ & $ 5.765 \pm 0.880 $ \\
\enddata
\tablerefs{The cloud's series number (Column 1), Galactic coordinates (Columns 2 and 3), distance (Columns 4) and boundary extinction (Columns 5) retrieved from Table 1 of \citet{Chen2020_catalogue}.}
\tablecomments{A machine-readable version of the full Table \ref{tab:catalog} is available.}
\label{tab:catalog}
\end{deluxetable*}

==> possibly_correlated.tex <==
\begin{figure*}[htb!]
\gridline{\fig{figures/MC_10}{0.33\textwidth}{(1) Cloud 10}
          \fig{figures/MC_12}{0.33\textwidth}{(2) Cloud 12}
          \fig{figures/MC_14}{0.33\textwidth}{(3) Cloud 14}}
\gridline{\fig{figures/MC_25}{0.33\textwidth}{(4) Cloud 25}
          \fig{figures/MC_28}{0.33\textwidth}{(5) Cloud 28}
          \fig{figures/MC_32}{0.33\textwidth}{(6) Cloud 32}}
\gridline{\fig{figures/MC_38}{0.33\textwidth}{(7) Cloud 38}
          \fig{figures/MC_39}{0.33\textwidth}{(8) Cloud 39}
          \fig{figures/MC_41}{0.33\textwidth}{(9) Cloud 41}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_43}{0.33\textwidth}{(1) Cloud 43}
          \fig{figures/MC_47}{0.33\textwidth}{(2) Cloud 47}
          \fig{figures/MC_49}{0.33\textwidth}{(3) Cloud 49}}
\gridline{\fig{figures/MC_50}{0.33\textwidth}{(4) Cloud 50}
          \fig{figures/MC_51}{0.33\textwidth}{(5) Cloud 51}
          \fig{figures/MC_53}{0.33\textwidth}{(6) Cloud 53}}
\gridline{\fig{figures/MC_55}{0.33\textwidth}{(7) Cloud 55}
          \fig{figures/MC_56}{0.33\textwidth}{(8) Cloud 56}
          \fig{figures/MC_58}{0.33\textwidth}{(9) Cloud 58}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_59}{0.33\textwidth}{(1) Cloud 59}
          \fig{figures/MC_62}{0.33\textwidth}{(2) Cloud 62}
          \fig{figures/MC_63}{0.33\textwidth}{(3) Cloud 63}}
\gridline{\fig{figures/MC_64}{0.33\textwidth}{(4) Cloud 64}
          \fig{figures/MC_65}{0.33\textwidth}{(5) Cloud 65}
          \fig{figures/MC_66}{0.33\textwidth}{(6) Cloud 66}}
\gridline{\fig{figures/MC_70}{0.33\textwidth}{(7) Cloud 70}
          \fig{figures/MC_73}{0.33\textwidth}{(8) Cloud 73}
          \fig{figures/MC_74}{0.33\textwidth}{(9) Cloud 74}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_75}{0.33\textwidth}{(1) Cloud 75}
          \fig{figures/MC_77}{0.33\textwidth}{(2) Cloud 77}
          \fig{figures/MC_79}{0.33\textwidth}{(3) Cloud 79}}
\gridline{\fig{figures/MC_80}{0.33\textwidth}{(4) Cloud 80}
          \fig{figures/MC_82}{0.33\textwidth}{(5) Cloud 82}
          \fig{figures/MC_83}{0.33\textwidth}{(6) Cloud 83}}
\gridline{\fig{figures/MC_84}{0.33\textwidth}{(7) Cloud 84}
          \fig{figures/MC_85}{0.33\textwidth}{(8) Cloud 85}
          \fig{figures/MC_86}{0.33\textwidth}{(9) Cloud 86}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_87}{0.33\textwidth}{(1) Cloud 87}
          \fig{figures/MC_88}{0.33\textwidth}{(2) Cloud 88}
          \fig{figures/MC_91}{0.33\textwidth}{(3) Cloud 91}}
\gridline{\fig{figures/MC_92}{0.33\textwidth}{(4) Cloud 92}
          \fig{figures/MC_93}{0.33\textwidth}{(5) Cloud 93}
          \fig{figures/MC_94}{0.33\textwidth}{(6) Cloud 94}}
\gridline{\fig{figures/MC_96}{0.33\textwidth}{(7) Cloud 96}
          \fig{figures/MC_99}{0.33\textwidth}{(8) Cloud 99}
          \fig{figures/MC_100}{0.33\textwidth}{(9) Cloud 100}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_101}{0.33\textwidth}{(1) Cloud 101}
          \fig{figures/MC_102}{0.33\textwidth}{(2) Cloud 102}
          \fig{figures/MC_103}{0.33\textwidth}{(3) Cloud 103}}
\gridline{\fig{figures/MC_104}{0.33\textwidth}{(4) Cloud 104}
          \fig{figures/MC_105}{0.33\textwidth}{(5) Cloud 105}
          \fig{figures/MC_108}{0.33\textwidth}{(6) Cloud 108}}
\gridline{\fig{figures/MC_109}{0.33\textwidth}{(7) Cloud 109}
          \fig{figures/MC_110}{0.33\textwidth}{(8) Cloud 110}
          \fig{figures/MC_112}{0.33\textwidth}{(9) Cloud 112}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_115}{0.33\textwidth}{(1) Cloud 115}
          \fig{figures/MC_118}{0.33\textwidth}{(2) Cloud 118}
          \fig{figures/MC_119}{0.33\textwidth}{(3) Cloud 119}}
\gridline{\fig{figures/MC_120}{0.33\textwidth}{(4) Cloud 120}
          \fig{figures/MC_121}{0.33\textwidth}{(5) Cloud 121}
          \fig{figures/MC_122}{0.33\textwidth}{(6) Cloud 122}}
\gridline{\fig{figures/MC_123}{0.33\textwidth}{(7) Cloud 123}
          \fig{figures/MC_125}{0.33\textwidth}{(8) Cloud 125}
          \fig{figures/MC_127}{0.33\textwidth}{(9) Cloud 127}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_128}{0.33\textwidth}{(1) Cloud 128}
          \fig{figures/MC_129}{0.33\textwidth}{(2) Cloud 129}
          \fig{figures/MC_130}{0.33\textwidth}{(3) Cloud 130}}
\gridline{\fig{figures/MC_131}{0.33\textwidth}{(4) Cloud 131}
          \fig{figures/MC_133}{0.33\textwidth}{(5) Cloud 133}
          \fig{figures/MC_134}{0.33\textwidth}{(6) Cloud 134}}
\gridline{\fig{figures/MC_135}{0.33\textwidth}{(7) Cloud 135}
          \fig{figures/MC_136}{0.33\textwidth}{(8) Cloud 136}
          \fig{figures/MC_141}{0.33\textwidth}{(9) Cloud 141}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_142}{0.33\textwidth}{(1) Cloud 142}
          \fig{figures/MC_144}{0.33\textwidth}{(2) Cloud 144}
          \fig{figures/MC_146}{0.33\textwidth}{(3) Cloud 146}}
\gridline{\fig{figures/MC_149}{0.33\textwidth}{(4) Cloud 149}
          \fig{figures/MC_152}{0.33\textwidth}{(5) Cloud 152}
          \fig{figures/MC_153}{0.33\textwidth}{(6) Cloud 153}}
\gridline{\fig{figures/MC_154}{0.33\textwidth}{(7) Cloud 154}
          \fig{figures/MC_156}{0.33\textwidth}{(8) Cloud 156}
          \fig{figures/MC_158}{0.33\textwidth}{(9) Cloud 158}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_159}{0.33\textwidth}{(1) Cloud 159}
          \fig{figures/MC_161}{0.33\textwidth}{(2) Cloud 161}
          \fig{figures/MC_163}{0.33\textwidth}{(3) Cloud 163}}
\gridline{\fig{figures/MC_164}{0.33\textwidth}{(4) Cloud 164}
          \fig{figures/MC_169}{0.33\textwidth}{(5) Cloud 169}
          \fig{figures/MC_171}{0.33\textwidth}{(6) Cloud 171}}
\gridline{\fig{figures/MC_172}{0.33\textwidth}{(7) Cloud 172}
          \fig{figures/MC_173}{0.33\textwidth}{(8) Cloud 173}
          \fig{figures/MC_177}{0.33\textwidth}{(9) Cloud 177}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_179}{0.33\textwidth}{(1) Cloud 179}
          \fig{figures/MC_182}{0.33\textwidth}{(2) Cloud 182}
          \fig{figures/MC_187}{0.33\textwidth}{(3) Cloud 187}}
\gridline{\fig{figures/MC_188}{0.33\textwidth}{(4) Cloud 188}
          \fig{figures/MC_189}{0.33\textwidth}{(5) Cloud 189}
          \fig{figures/MC_192}{0.33\textwidth}{(6) Cloud 192}}
\gridline{\fig{figures/MC_193}{0.33\textwidth}{(7) Cloud 193}
          \fig{figures/MC_195}{0.33\textwidth}{(8) Cloud 195}
          \fig{figures/MC_198}{0.33\textwidth}{(9) Cloud 198}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_199}{0.33\textwidth}{(1) Cloud 199}
          \fig{figures/MC_200}{0.33\textwidth}{(2) Cloud 200}
          \fig{figures/MC_202}{0.33\textwidth}{(3) Cloud 202}}
\gridline{\fig{figures/MC_205}{0.33\textwidth}{(4) Cloud 205}
          \fig{figures/MC_206}{0.33\textwidth}{(5) Cloud 206}
          \fig{figures/MC_207}{0.33\textwidth}{(6) Cloud 207}}
\gridline{\fig{figures/MC_209}{0.33\textwidth}{(7) Cloud 209}
          \fig{figures/MC_212}{0.33\textwidth}{(8) Cloud 212}
          \fig{figures/MC_213}{0.33\textwidth}{(9) Cloud 213}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_214}{0.33\textwidth}{(1) Cloud 214}
          \fig{figures/MC_215}{0.33\textwidth}{(2) Cloud 215}
          \fig{figures/MC_216}{0.33\textwidth}{(3) Cloud 216}}
\gridline{\fig{figures/MC_217}{0.33\textwidth}{(4) Cloud 217}
          \fig{figures/MC_218}{0.33\textwidth}{(5) Cloud 218}
          \fig{figures/MC_219}{0.33\textwidth}{(6) Cloud 219}}
\gridline{\fig{figures/MC_220}{0.33\textwidth}{(7) Cloud 220}
          \fig{figures/MC_221}{0.33\textwidth}{(8) Cloud 221}
          \fig{figures/MC_222}{0.33\textwidth}{(9) Cloud 222}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_223}{0.33\textwidth}{(1) Cloud 223}
          \fig{figures/MC_227}{0.33\textwidth}{(2) Cloud 227}
          \fig{figures/MC_228}{0.33\textwidth}{(3) Cloud 228}}
\gridline{\fig{figures/MC_229}{0.33\textwidth}{(4) Cloud 229}
          \fig{figures/MC_232}{0.33\textwidth}{(5) Cloud 232}
          \fig{figures/MC_233}{0.33\textwidth}{(6) Cloud 233}}
\gridline{\fig{figures/MC_235}{0.33\textwidth}{(7) Cloud 235}
          \fig{figures/MC_237}{0.33\textwidth}{(8) Cloud 237}
          \fig{figures/MC_240}{0.33\textwidth}{(9) Cloud 240}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_241}{0.33\textwidth}{(1) Cloud 241}
          \fig{figures/MC_244}{0.33\textwidth}{(2) Cloud 244}
          \fig{figures/MC_245}{0.33\textwidth}{(3) Cloud 245}}
\gridline{\fig{figures/MC_246}{0.33\textwidth}{(4) Cloud 246}
          \fig{figures/MC_248}{0.33\textwidth}{(5) Cloud 248}
          \fig{figures/MC_251}{0.33\textwidth}{(6) Cloud 251}}
\gridline{\fig{figures/MC_253}{0.33\textwidth}{(7) Cloud 253}
          \fig{figures/MC_254}{0.33\textwidth}{(8) Cloud 254}
          \fig{figures/MC_255}{0.33\textwidth}{(9) Cloud 255}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_256}{0.33\textwidth}{(1) Cloud 256}
          \fig{figures/MC_257}{0.33\textwidth}{(2) Cloud 257}
          \fig{figures/MC_258}{0.33\textwidth}{(3) Cloud 258}}
\gridline{\fig{figures/MC_259}{0.33\textwidth}{(4) Cloud 259}
          \fig{figures/MC_260}{0.33\textwidth}{(5) Cloud 260}
          \fig{figures/MC_261}{0.33\textwidth}{(6) Cloud 261}}
\gridline{\fig{figures/MC_264}{0.33\textwidth}{(7) Cloud 264}
          \fig{figures/MC_265}{0.33\textwidth}{(8) Cloud 265}
          \fig{figures/MC_268}{0.33\textwidth}{(9) Cloud 268}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_269}{0.33\textwidth}{(1) Cloud 269}
          \fig{figures/MC_270}{0.33\textwidth}{(2) Cloud 270}
          \fig{figures/MC_273}{0.33\textwidth}{(3) Cloud 273}}
\gridline{\fig{figures/MC_274}{0.33\textwidth}{(4) Cloud 274}
          \fig{figures/MC_275}{0.33\textwidth}{(5) Cloud 275}
          \fig{figures/MC_277}{0.33\textwidth}{(6) Cloud 277}}
\gridline{\fig{figures/MC_278}{0.33\textwidth}{(7) Cloud 278}
          \fig{figures/MC_279}{0.33\textwidth}{(8) Cloud 279}
          \fig{figures/MC_280}{0.33\textwidth}{(9) Cloud 280}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_281}{0.33\textwidth}{(1) Cloud 281}
          \fig{figures/MC_283}{0.33\textwidth}{(2) Cloud 283}
          \fig{figures/MC_284}{0.33\textwidth}{(3) Cloud 284}}
\gridline{\fig{figures/MC_286}{0.33\textwidth}{(4) Cloud 286}
          \fig{figures/MC_287}{0.33\textwidth}{(5) Cloud 287}
          \fig{figures/MC_289}{0.33\textwidth}{(6) Cloud 289}}
\gridline{\fig{figures/MC_292}{0.33\textwidth}{(7) Cloud 292}
          \fig{figures/MC_297}{0.33\textwidth}{(8) Cloud 297}
          \fig{figures/MC_298}{0.33\textwidth}{(9) Cloud 298}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_299}{0.33\textwidth}{(1) Cloud 299}
          \fig{figures/MC_300}{0.33\textwidth}{(2) Cloud 300}
          \fig{figures/MC_301}{0.33\textwidth}{(3) Cloud 301}}
\gridline{\fig{figures/MC_302}{0.33\textwidth}{(4) Cloud 302}
          \fig{figures/MC_304}{0.33\textwidth}{(5) Cloud 304}
          \fig{figures/MC_308}{0.33\textwidth}{(6) Cloud 308}}
\gridline{\fig{figures/MC_309}{0.33\textwidth}{(7) Cloud 309}
          \fig{figures/MC_310}{0.33\textwidth}{(8) Cloud 310}
          \fig{figures/MC_312}{0.33\textwidth}{(9) Cloud 312}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_313}{0.33\textwidth}{(1) Cloud 313}
          \fig{figures/MC_315}{0.33\textwidth}{(2) Cloud 315}
          \fig{figures/MC_316}{0.33\textwidth}{(3) Cloud 316}}
\gridline{\fig{figures/MC_317}{0.33\textwidth}{(4) Cloud 317}
          \fig{figures/MC_318}{0.33\textwidth}{(5) Cloud 318}
          \fig{figures/MC_319}{0.33\textwidth}{(6) Cloud 319}}
\gridline{\fig{figures/MC_321}{0.33\textwidth}{(7) Cloud 321}
          \fig{figures/MC_322}{0.33\textwidth}{(8) Cloud 322}
          \fig{figures/MC_323}{0.33\textwidth}{(9) Cloud 323}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_324}{0.33\textwidth}{(1) Cloud 324}
          \fig{figures/MC_326}{0.33\textwidth}{(2) Cloud 326}
          \fig{figures/MC_327}{0.33\textwidth}{(3) Cloud 327}}
\gridline{\fig{figures/MC_328}{0.33\textwidth}{(4) Cloud 328}
          \fig{figures/MC_330}{0.33\textwidth}{(5) Cloud 330}
          \fig{figures/MC_331}{0.33\textwidth}{(6) Cloud 331}}
\gridline{\fig{figures/MC_333}{0.33\textwidth}{(7) Cloud 333}
          \fig{figures/MC_334}{0.33\textwidth}{(8) Cloud 334}
          \fig{figures/MC_335}{0.33\textwidth}{(9) Cloud 335}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_336}{0.33\textwidth}{(1) Cloud 336}
          \fig{figures/MC_337}{0.33\textwidth}{(2) Cloud 337}
          \fig{figures/MC_339}{0.33\textwidth}{(3) Cloud 339}}
\gridline{\fig{figures/MC_343}{0.33\textwidth}{(4) Cloud 343}
          \fig{figures/MC_344}{0.33\textwidth}{(5) Cloud 344}
          \fig{figures/MC_345}{0.33\textwidth}{(6) Cloud 345}}
\gridline{\fig{figures/MC_347}{0.33\textwidth}{(7) Cloud 347}
          \fig{figures/MC_349}{0.33\textwidth}{(8) Cloud 349}
          \fig{figures/MC_353}{0.33\textwidth}{(9) Cloud 353}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_359}{0.33\textwidth}{(1) Cloud 359}
          \fig{figures/MC_361}{0.33\textwidth}{(2) Cloud 361}
          \fig{figures/MC_363}{0.33\textwidth}{(3) Cloud 363}}
\gridline{\fig{figures/MC_365}{0.33\textwidth}{(4) Cloud 365}
          \fig{figures/MC_366}{0.33\textwidth}{(5) Cloud 366}
          \fig{figures/MC_367}{0.33\textwidth}{(6) Cloud 367}}
\gridline{\fig{figures/MC_369}{0.33\textwidth}{(7) Cloud 369}
          \fig{figures/MC_371}{0.33\textwidth}{(8) Cloud 371}
          \fig{figures/MC_374}{0.33\textwidth}{(9) Cloud 374}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_375}{0.33\textwidth}{(1) Cloud 375}
          \fig{figures/MC_377}{0.33\textwidth}{(2) Cloud 377}
          \fig{figures/MC_379}{0.33\textwidth}{(3) Cloud 379}}
\gridline{\fig{figures/MC_381}{0.33\textwidth}{(4) Cloud 381}
          \fig{figures/MC_383}{0.33\textwidth}{(5) Cloud 383}
          \fig{figures/MC_384}{0.33\textwidth}{(6) Cloud 384}}
\gridline{\fig{figures/MC_385}{0.33\textwidth}{(7) Cloud 385}
          \fig{figures/MC_386}{0.33\textwidth}{(8) Cloud 386}
          \fig{figures/MC_387}{0.33\textwidth}{(9) Cloud 387}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_388}{0.33\textwidth}{(1) Cloud 388}
          \fig{figures/MC_390}{0.33\textwidth}{(2) Cloud 390}
          \fig{figures/MC_391}{0.33\textwidth}{(3) Cloud 391}}
\gridline{\fig{figures/MC_393}{0.33\textwidth}{(4) Cloud 393}
          \fig{figures/MC_394}{0.33\textwidth}{(5) Cloud 394}
          \fig{figures/MC_395}{0.33\textwidth}{(6) Cloud 395}}
\gridline{\fig{figures/MC_399}{0.33\textwidth}{(7) Cloud 399}
          \fig{figures/MC_400}{0.33\textwidth}{(8) Cloud 400}
          \fig{figures/MC_402}{0.33\textwidth}{(9) Cloud 402}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_404}{0.33\textwidth}{(1) Cloud 404}
          \fig{figures/MC_405}{0.33\textwidth}{(2) Cloud 405}
          \fig{figures/MC_406}{0.33\textwidth}{(3) Cloud 406}}
\gridline{\fig{figures/MC_408}{0.33\textwidth}{(4) Cloud 408}
          \fig{figures/MC_409}{0.33\textwidth}{(5) Cloud 409}
          \fig{figures/MC_410}{0.33\textwidth}{(6) Cloud 410}}
\gridline{\fig{figures/MC_411}{0.33\textwidth}{(7) Cloud 411}
          \fig{figures/MC_412}{0.33\textwidth}{(8) Cloud 412}
          \fig{figures/MC_413}{0.33\textwidth}{(9) Cloud 413}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_414}{0.33\textwidth}{(1) Cloud 414}
          \fig{figures/MC_416}{0.33\textwidth}{(2) Cloud 416}
          \fig{figures/MC_417}{0.33\textwidth}{(3) Cloud 417}}
\gridline{\fig{figures/MC_419}{0.33\textwidth}{(4) Cloud 419}
          \fig{figures/MC_420}{0.33\textwidth}{(5) Cloud 420}
          \fig{figures/MC_421}{0.33\textwidth}{(6) Cloud 421}}
\gridline{\fig{figures/MC_423}{0.33\textwidth}{(7) Cloud 423}
          \fig{figures/MC_426}{0.33\textwidth}{(8) Cloud 426}
          \fig{figures/MC_429}{0.33\textwidth}{(9) Cloud 429}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_430}{0.33\textwidth}{(1) Cloud 430}
          \fig{figures/MC_431}{0.33\textwidth}{(2) Cloud 431}
          \fig{figures/MC_432}{0.33\textwidth}{(3) Cloud 432}}
\gridline{\fig{figures/MC_433}{0.33\textwidth}{(4) Cloud 433}
          \fig{figures/MC_435}{0.33\textwidth}{(5) Cloud 435}
          \fig{figures/MC_436}{0.33\textwidth}{(6) Cloud 436}}
\gridline{\fig{figures/MC_437}{0.33\textwidth}{(7) Cloud 437}
          \fig{figures/MC_439}{0.33\textwidth}{(8) Cloud 439}
          \fig{figures/MC_440}{0.33\textwidth}{(9) Cloud 440}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_442}{0.33\textwidth}{(1) Cloud 442}
          \fig{figures/MC_443}{0.33\textwidth}{(2) Cloud 443}
          \fig{figures/MC_444}{0.33\textwidth}{(3) Cloud 444}}
\gridline{\fig{figures/MC_446}{0.33\textwidth}{(4) Cloud 446}
          \fig{figures/MC_452}{0.33\textwidth}{(5) Cloud 452}
          \fig{figures/MC_454}{0.33\textwidth}{(6) Cloud 454}}
\gridline{\fig{figures/MC_456}{0.33\textwidth}{(7) Cloud 456}
          \fig{figures/MC_457}{0.33\textwidth}{(8) Cloud 457}
          \fig{figures/MC_458}{0.33\textwidth}{(9) Cloud 458}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_459}{0.33\textwidth}{(1) Cloud 459}
          \fig{figures/MC_460}{0.33\textwidth}{(2) Cloud 460}
          \fig{figures/MC_462}{0.33\textwidth}{(3) Cloud 462}}
\gridline{\fig{figures/MC_463}{0.33\textwidth}{(4) Cloud 463}
          \fig{figures/MC_464}{0.33\textwidth}{(5) Cloud 464}
          \fig{figures/MC_465}{0.33\textwidth}{(6) Cloud 465}}
\gridline{\fig{figures/MC_466}{0.33\textwidth}{(7) Cloud 466}
          \fig{figures/MC_468}{0.33\textwidth}{(8) Cloud 468}
          \fig{figures/MC_469}{0.33\textwidth}{(9) Cloud 469}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_470}{0.33\textwidth}{(1) Cloud 470}
          \fig{figures/MC_471}{0.33\textwidth}{(2) Cloud 471}
          \fig{figures/MC_472}{0.33\textwidth}{(3) Cloud 472}}
\gridline{\fig{figures/MC_473}{0.33\textwidth}{(4) Cloud 473}
          \fig{figures/MC_474}{0.33\textwidth}{(5) Cloud 474}
          \fig{figures/MC_477}{0.33\textwidth}{(6) Cloud 477}}
\gridline{\fig{figures/MC_478}{0.33\textwidth}{(7) Cloud 478}
          \fig{figures/MC_479}{0.33\textwidth}{(8) Cloud 479}
          \fig{figures/MC_486}{0.33\textwidth}{(9) Cloud 486}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_487}{0.33\textwidth}{(1) Cloud 487}
          \fig{figures/MC_491}{0.33\textwidth}{(2) Cloud 491}
          \fig{figures/MC_493}{0.33\textwidth}{(3) Cloud 493}}
\gridline{\fig{figures/MC_495}{0.33\textwidth}{(4) Cloud 495}
          \fig{figures/MC_496}{0.33\textwidth}{(5) Cloud 496}
          \fig{figures/MC_497}{0.33\textwidth}{(6) Cloud 497}}
\gridline{\fig{figures/MC_498}{0.33\textwidth}{(7) Cloud 498}
          \fig{figures/MC_499}{0.33\textwidth}{(8) Cloud 499}
          \fig{figures/MC_501}{0.33\textwidth}{(9) Cloud 501}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_504}{0.33\textwidth}{(1) Cloud 504}
          \fig{figures/MC_505}{0.33\textwidth}{(2) Cloud 505}
          \fig{figures/MC_507}{0.33\textwidth}{(3) Cloud 507}}
\gridline{\fig{figures/MC_508}{0.33\textwidth}{(4) Cloud 508}
          \fig{figures/MC_510}{0.33\textwidth}{(5) Cloud 510}
          \fig{figures/MC_511}{0.33\textwidth}{(6) Cloud 511}}
\gridline{\fig{figures/MC_512}{0.33\textwidth}{(7) Cloud 512}
          \fig{figures/MC_514}{0.33\textwidth}{(8) Cloud 514}
          \fig{figures/MC_516}{0.33\textwidth}{(9) Cloud 516}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_517}{0.33\textwidth}{(1) Cloud 517}
          \fig{figures/MC_518}{0.33\textwidth}{(2) Cloud 518}
          \fig{figures/MC_519}{0.33\textwidth}{(3) Cloud 519}}
\gridline{\fig{figures/MC_520}{0.33\textwidth}{(4) Cloud 520}
          \fig{figures/MC_524}{0.33\textwidth}{(5) Cloud 524}
          \fig{figures/MC_525}{0.33\textwidth}{(6) Cloud 525}}
\gridline{\fig{figures/MC_526}{0.33\textwidth}{(7) Cloud 526}
          \fig{figures/MC_527}{0.33\textwidth}{(8) Cloud 527}
          \fig{figures/MC_528}{0.33\textwidth}{(9) Cloud 528}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_529}{0.33\textwidth}{(1) Cloud 529}
          \fig{figures/MC_530}{0.33\textwidth}{(2) Cloud 530}
          \fig{figures/MC_532}{0.33\textwidth}{(3) Cloud 532}}
\gridline{\fig{figures/MC_534}{0.33\textwidth}{(4) Cloud 534}
          \fig{figures/MC_535}{0.33\textwidth}{(5) Cloud 535}
          \fig{figures/MC_536}{0.33\textwidth}{(6) Cloud 536}}
\gridline{\fig{figures/MC_539}{0.33\textwidth}{(7) Cloud 539}
          \fig{figures/MC_540}{0.33\textwidth}{(8) Cloud 540}
          \fig{figures/MC_541}{0.33\textwidth}{(9) Cloud 541}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_542}{0.33\textwidth}{(1) Cloud 542}
          \fig{figures/MC_544}{0.33\textwidth}{(2) Cloud 544}
          \fig{figures/MC_545}{0.33\textwidth}{(3) Cloud 545}}
\gridline{\fig{figures/MC_546}{0.33\textwidth}{(4) Cloud 546}
          \fig{figures/MC_547}{0.33\textwidth}{(5) Cloud 547}
          \fig{figures/MC_549}{0.33\textwidth}{(6) Cloud 549}}
\gridline{\fig{figures/MC_550}{0.33\textwidth}{(7) Cloud 550}
          \fig{figures/MC_551}{0.33\textwidth}{(8) Cloud 551}
          \fig{figures/MC_552}{0.33\textwidth}{(9) Cloud 552}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_554}{0.33\textwidth}{(1) Cloud 554}
          \fig{figures/MC_555}{0.33\textwidth}{(2) Cloud 555}
          \fig{figures/MC_556}{0.33\textwidth}{(3) Cloud 556}}
\gridline{\fig{figures/MC_557}{0.33\textwidth}{(4) Cloud 557}
          \fig{figures/MC_559}{0.33\textwidth}{(5) Cloud 559}
          \fig{figures/MC_560}{0.33\textwidth}{(6) Cloud 560}}
\gridline{\fig{figures/MC_562}{0.33\textwidth}{(7) Cloud 562}
          \fig{figures/MC_565}{0.33\textwidth}{(8) Cloud 565}
          \fig{figures/MC_566}{0.33\textwidth}{(9) Cloud 566}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

==> strongly_correlated.tex <==
\begin{figure*}[htb!]
\gridline{\fig{figures/MC_1}{0.33\textwidth}{(1) Cloud 1}
          \fig{figures/MC_2}{0.33\textwidth}{(2) Cloud 2}
          \fig{figures/MC_3}{0.33\textwidth}{(3) Cloud 3}}
\gridline{\fig{figures/MC_4}{0.33\textwidth}{(4) Cloud 4}
          \fig{figures/MC_13}{0.33\textwidth}{(5) Cloud 13}
          \fig{figures/MC_27}{0.33\textwidth}{(6) Cloud 27}}
\gridline{\fig{figures/MC_29}{0.33\textwidth}{(7) Cloud 29}
          \fig{figures/MC_36}{0.33\textwidth}{(8) Cloud 36}
          \fig{figures/MC_60}{0.33\textwidth}{(9) Cloud 60}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_61}{0.33\textwidth}{(1) Cloud 61}
          \fig{figures/MC_67}{0.33\textwidth}{(2) Cloud 67}
          \fig{figures/MC_68}{0.33\textwidth}{(3) Cloud 68}}
\gridline{\fig{figures/MC_71}{0.33\textwidth}{(4) Cloud 71}
          \fig{figures/MC_78}{0.33\textwidth}{(5) Cloud 78}
          \fig{figures/MC_89}{0.33\textwidth}{(6) Cloud 89}}
\gridline{\fig{figures/MC_90}{0.33\textwidth}{(7) Cloud 90}
          \fig{figures/MC_95}{0.33\textwidth}{(8) Cloud 95}
          \fig{figures/MC_97}{0.33\textwidth}{(9) Cloud 97}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_106}{0.33\textwidth}{(1) Cloud 106}
          \fig{figures/MC_111}{0.33\textwidth}{(2) Cloud 111}
          \fig{figures/MC_114}{0.33\textwidth}{(3) Cloud 114}}
\gridline{\fig{figures/MC_116}{0.33\textwidth}{(4) Cloud 116}
          \fig{figures/MC_117}{0.33\textwidth}{(5) Cloud 117}
          \fig{figures/MC_137}{0.33\textwidth}{(6) Cloud 137}}
\gridline{\fig{figures/MC_138}{0.33\textwidth}{(7) Cloud 138}
          \fig{figures/MC_139}{0.33\textwidth}{(8) Cloud 139}
          \fig{figures/MC_140}{0.33\textwidth}{(9) Cloud 140}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_143}{0.33\textwidth}{(1) Cloud 143}
          \fig{figures/MC_151}{0.33\textwidth}{(2) Cloud 151}
          \fig{figures/MC_155}{0.33\textwidth}{(3) Cloud 155}}
\gridline{\fig{figures/MC_157}{0.33\textwidth}{(4) Cloud 157}
          \fig{figures/MC_166}{0.33\textwidth}{(5) Cloud 166}
          \fig{figures/MC_170}{0.33\textwidth}{(6) Cloud 170}}
\gridline{\fig{figures/MC_174}{0.33\textwidth}{(7) Cloud 174}
          \fig{figures/MC_176}{0.33\textwidth}{(8) Cloud 176}
          \fig{figures/MC_178}{0.33\textwidth}{(9) Cloud 178}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_180}{0.33\textwidth}{(1) Cloud 180}
          \fig{figures/MC_186}{0.33\textwidth}{(2) Cloud 186}
          \fig{figures/MC_190}{0.33\textwidth}{(3) Cloud 190}}
\gridline{\fig{figures/MC_191}{0.33\textwidth}{(4) Cloud 191}
          \fig{figures/MC_194}{0.33\textwidth}{(5) Cloud 194}
          \fig{figures/MC_196}{0.33\textwidth}{(6) Cloud 196}}
\gridline{\fig{figures/MC_197}{0.33\textwidth}{(7) Cloud 197}
          \fig{figures/MC_203}{0.33\textwidth}{(8) Cloud 203}
          \fig{figures/MC_204}{0.33\textwidth}{(9) Cloud 204}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_208}{0.33\textwidth}{(1) Cloud 208}
          \fig{figures/MC_210}{0.33\textwidth}{(2) Cloud 210}
          \fig{figures/MC_211}{0.33\textwidth}{(3) Cloud 211}}
\gridline{\fig{figures/MC_224}{0.33\textwidth}{(4) Cloud 224}
          \fig{figures/MC_225}{0.33\textwidth}{(5) Cloud 225}
          \fig{figures/MC_230}{0.33\textwidth}{(6) Cloud 230}}
\gridline{\fig{figures/MC_231}{0.33\textwidth}{(7) Cloud 231}
          \fig{figures/MC_234}{0.33\textwidth}{(8) Cloud 234}
          \fig{figures/MC_239}{0.33\textwidth}{(9) Cloud 239}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_242}{0.33\textwidth}{(1) Cloud 242}
          \fig{figures/MC_243}{0.33\textwidth}{(2) Cloud 243}
          \fig{figures/MC_247}{0.33\textwidth}{(3) Cloud 247}}
\gridline{\fig{figures/MC_249}{0.33\textwidth}{(4) Cloud 249}
          \fig{figures/MC_250}{0.33\textwidth}{(5) Cloud 250}
          \fig{figures/MC_252}{0.33\textwidth}{(6) Cloud 252}}
\gridline{\fig{figures/MC_262}{0.33\textwidth}{(7) Cloud 262}
          \fig{figures/MC_263}{0.33\textwidth}{(8) Cloud 263}
          \fig{figures/MC_266}{0.33\textwidth}{(9) Cloud 266}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_267}{0.33\textwidth}{(1) Cloud 267}
          \fig{figures/MC_271}{0.33\textwidth}{(2) Cloud 271}
          \fig{figures/MC_272}{0.33\textwidth}{(3) Cloud 272}}
\gridline{\fig{figures/MC_290}{0.33\textwidth}{(4) Cloud 290}
          \fig{figures/MC_291}{0.33\textwidth}{(5) Cloud 291}
          \fig{figures/MC_294}{0.33\textwidth}{(6) Cloud 294}}
\gridline{\fig{figures/MC_296}{0.33\textwidth}{(7) Cloud 296}
          \fig{figures/MC_303}{0.33\textwidth}{(8) Cloud 303}
          \fig{figures/MC_305}{0.33\textwidth}{(9) Cloud 305}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_306}{0.33\textwidth}{(1) Cloud 306}
          \fig{figures/MC_307}{0.33\textwidth}{(2) Cloud 307}
          \fig{figures/MC_311}{0.33\textwidth}{(3) Cloud 311}}
\gridline{\fig{figures/MC_329}{0.33\textwidth}{(4) Cloud 329}
          \fig{figures/MC_332}{0.33\textwidth}{(5) Cloud 332}
          \fig{figures/MC_338}{0.33\textwidth}{(6) Cloud 338}}
\gridline{\fig{figures/MC_341}{0.33\textwidth}{(7) Cloud 341}
          \fig{figures/MC_346}{0.33\textwidth}{(8) Cloud 346}
          \fig{figures/MC_351}{0.33\textwidth}{(9) Cloud 351}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_352}{0.33\textwidth}{(1) Cloud 352}
          \fig{figures/MC_354}{0.33\textwidth}{(2) Cloud 354}
          \fig{figures/MC_355}{0.33\textwidth}{(3) Cloud 355}}
\gridline{\fig{figures/MC_356}{0.33\textwidth}{(4) Cloud 356}
          \fig{figures/MC_357}{0.33\textwidth}{(5) Cloud 357}
          \fig{figures/MC_364}{0.33\textwidth}{(6) Cloud 364}}
\gridline{\fig{figures/MC_368}{0.33\textwidth}{(7) Cloud 368}
          \fig{figures/MC_370}{0.33\textwidth}{(8) Cloud 370}
          \fig{figures/MC_372}{0.33\textwidth}{(9) Cloud 372}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_373}{0.33\textwidth}{(1) Cloud 373}
          \fig{figures/MC_378}{0.33\textwidth}{(2) Cloud 378}
          \fig{figures/MC_392}{0.33\textwidth}{(3) Cloud 392}}
\gridline{\fig{figures/MC_396}{0.33\textwidth}{(4) Cloud 396}
          \fig{figures/MC_397}{0.33\textwidth}{(5) Cloud 397}
          \fig{figures/MC_403}{0.33\textwidth}{(6) Cloud 403}}
\gridline{\fig{figures/MC_407}{0.33\textwidth}{(7) Cloud 407}
          \fig{figures/MC_415}{0.33\textwidth}{(8) Cloud 415}
          \fig{figures/MC_422}{0.33\textwidth}{(9) Cloud 422}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_427}{0.33\textwidth}{(1) Cloud 427}
          \fig{figures/MC_434}{0.33\textwidth}{(2) Cloud 434}
          \fig{figures/MC_438}{0.33\textwidth}{(3) Cloud 438}}
\gridline{\fig{figures/MC_450}{0.33\textwidth}{(4) Cloud 450}
          \fig{figures/MC_451}{0.33\textwidth}{(5) Cloud 451}
          \fig{figures/MC_453}{0.33\textwidth}{(6) Cloud 453}}
\gridline{\fig{figures/MC_455}{0.33\textwidth}{(7) Cloud 455}
          \fig{figures/MC_480}{0.33\textwidth}{(8) Cloud 480}
          \fig{figures/MC_494}{0.33\textwidth}{(9) Cloud 494}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_509}{0.33\textwidth}{(1) Cloud 509}
          \fig{figures/MC_533}{0.33\textwidth}{(2) Cloud 533}}
\gridline{\fig{figures/MC_548}{0.33\textwidth}{(3) Cloud 548}
          \fig{figures/MC_553}{0.33\textwidth}{(4) Cloud 553}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

==> uncorrelated.tex <==
\begin{figure*}[htb!]
\gridline{\fig{figures/MC_22}{0.33\textwidth}{(1) Cloud 22}
          \fig{figures/MC_23}{0.33\textwidth}{(2) Cloud 23}
          \fig{figures/MC_31}{0.33\textwidth}{(3) Cloud 31}}
\gridline{\fig{figures/MC_46}{0.33\textwidth}{(4) Cloud 46}
          \fig{figures/MC_48}{0.33\textwidth}{(5) Cloud 48}
          \fig{figures/MC_69}{0.33\textwidth}{(6) Cloud 69}}
\gridline{\fig{figures/MC_72}{0.33\textwidth}{(7) Cloud 72}
          \fig{figures/MC_76}{0.33\textwidth}{(8) Cloud 76}
          \fig{figures/MC_81}{0.33\textwidth}{(9) Cloud 81}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_98}{0.33\textwidth}{(1) Cloud 98}
          \fig{figures/MC_113}{0.33\textwidth}{(2) Cloud 113}
          \fig{figures/MC_132}{0.33\textwidth}{(3) Cloud 132}}
\gridline{\fig{figures/MC_145}{0.33\textwidth}{(4) Cloud 145}
          \fig{figures/MC_147}{0.33\textwidth}{(5) Cloud 147}
          \fig{figures/MC_175}{0.33\textwidth}{(6) Cloud 175}}
\gridline{\fig{figures/MC_325}{0.33\textwidth}{(7) Cloud 325}
          \fig{figures/MC_475}{0.33\textwidth}{(8) Cloud 475}
          \fig{figures/MC_484}{0.33\textwidth}{(9) Cloud 484}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage

\begin{figure*}[htb!]
\gridline{\fig{figures/MC_488}{0.33\textwidth}{(1) Cloud 488}
          \fig{figures/MC_492}{0.33\textwidth}{(2) Cloud 492}
          \fig{figures/MC_523}{0.33\textwidth}{(3) Cloud 523}}
\gridline{\fig{figures/MC_537}{0.33\textwidth}{(4) Cloud 537}
          \fig{figures/MC_558}{0.33\textwidth}{(5) Cloud 558}
          \fig{figures/MC_564}{0.33\textwidth}{(6) Cloud 564}}
\caption{See the caption of Figure \ref{fig:dust-CO well correlated} in the paper for details.}
\end{figure*}\clearpage


